Convergence of a time-stepping scheme to the free boundary in the supercooled Stefan problem

The supercooled Stefan problem and its variants describe the freezing of a supercooled liquid in physics, as well as the large system limits of systemic risk models in finance and of integrate-and-fire models in neuroscience. Adopting the physics terminology, the supercooled Stefan problem is known to feature a finite-time blow-up of the freezing rate for a wide range of initial temperature distributions in the liquid. Such a blow-up can result in a discontinuity of the liquid-solid boundary. In this paper, we prove that the natural Euler time-stepping scheme applied to a probabilistic formulation of the supercooled Stefan problem converges to the liquid-solid boundary of its physical solution globally in time, in the Skorokhod M1 topology. In the course of the proof, we give an explicit bound on the rate of local convergence for the time-stepping scheme. We also run numerical tests to compare our theoretical results to the practically observed convergence behavior.

==> arXiv v2/Section1.tex <==
%!TEX root =Main.tex

\section{Introduction}

The classical formulation of the one-dimensional one-phase Stefan problem (henceforth, simply Stefan problem), introduced by \textsc{Stefan} in \cite{Stefan1,Stefan2,Stefan3,Stefan4} (see also \cite{LC}), can be stated as follows: 
\begin{equation}\label{eq:Stefan}
	\begin{split}
		& \partial_t u = \frac{1}{2}\partial_{xx}u,\;\; x\ge \Lambda_t,\;\; t\ge 0, \\
		& u(0,x)=f(x),\;\; x\ge0 \quad\text{and}\quad u(t,\Lambda_t)=0,\;\; t\ge0, \\
		& \dot{\Lambda}_t = \frac{\alpha}{2}\partial_x u(t,\Lambda_t),\;\; t\ge0\quad\text{and}\quad\Lambda_0=0.
	\end{split}
\end{equation}
Hereby, the negative $-f$ of the given function $f:\,[0,\infty)\to\rr$ stands for the initial temperature distribution in a liquid relative to its equilibrium freezing point; $\Lambda_t$ is the unknown location of the liquid-solid boundary at time $t$; the negative $-u(t,\cdot)$ of the unknown function $u(t,\cdot):\,[\Lambda_t,\infty)\to\rr$ represents the temperature distribution in the liquid relative to its equilibrium freezing point at time $t$; and $\frac{2}{\alpha}>0$ is the density of latent heat when the heat capacity of the liquid is normalized to $2$ and its thermal conductivity to $1$. We consider the Stefan problem \eqref{eq:Stefan} in the \textit{supercooled} regime, i.e., when $f\ge0$.  

\medskip

As first observed by \textsc{Sherman} in \cite{Sher}, classical solutions of the supercooled Stefan problem can exhibit a finite-time blow-up, in the sense that $\lim_{t\uparrow t_*} \dot{\Lambda}_t=\infty$ for some $t_*\in(0,\infty)$. Subsequently, much attention has been devoted to the construction of classical solutions to \eqref{eq:Stefan} on $[0,t_*)$, to the distinction between the cases $t_*<\infty$ and $t_*=\infty$ in terms of the initial condition $f$ (see \cite{FP1,FP2,DF,HOL,LO,FPHO} and the references therein), and to the regularization of \eqref{eq:Stefan} when $t_*<\infty$ (see \cite{Vis,DHOX,FPHO,HX,Wei} and the references therein). 

\medskip

More recently, it has been discovered in \cite{NS1} that (a variant of) \eqref{eq:Stefan} admits a probabilistic reformulation (see also \cite[Section 1.2]{DIRT2} for a related discussion). Indeed, suppose that $\|f\|_{L^1([0,\infty))}=1$, let $X_{0-}$ be a random variable with the probability density $f$, and consider the problem of finding a non-decreasing function $\Lambda$ such that the stochastic process 
\begin{equation}\label{eq::init1}
	X_t = X_{0-} + B_t - \Lambda_t,\;\; t\ge 0 
\end{equation}
satisfies the constraint
\begin{equation}\label{eq::init2}
	\Lambda_t = \alpha\pp\Big(\inf_{0\le s\le t} X_s \le 0\Big),\;\;t\ge 0, 
\end{equation}
where $B$ is a standard Brownian motion independent of $X_{0-}$. Assuming that $f$ belongs to the Sobolev space $W^1_2([0,\infty))$ and that $f(0)=0$,  there exists a $T\in(0,\infty)$ and a solution $\Lambda$ of \eqref{eq::init1}--\eqref{eq::init2} on $[0,T]$ with $\dot{\Lambda}\in L^2([0,T])$; moreover,  with $\tau:=\inf\{t\ge0:\,X_t\le 0\}$, the densities $p(t,\cdot)$, $t\in[0,T]$ of $X_t\,\mathbf{1}_{\{\tau>t\}}$, $t\in[0,T]$ on $(0,\infty)$ form the unique solution of
\begin{equation}\label{p_PDE}
	\begin{split}
		& \partial_t p=\frac{1}{2}\partial_{xx}p+\dot{\Lambda}_t\partial_x p,\;\;x\ge0,\;\;t\in[0,T], \\ 
	 	& p(0,x)=f(x),\;\; x\ge 0\quad\text{and}\quad p(t,0)=0,\;\;t\in[0,T], \\
		& \dot{\Lambda}_t=\frac{\alpha}{2}\partial_x p(t,0),\;\;t\in[0,T]\quad\text{and}\quad\Lambda_0=0
	\end{split}
\end{equation}
in the Sobolev space $W^{1,2}_2([0,T]\times[0,\infty))$ (cf.~\cite[Propositions 4.1, 4.2]{NS1}), i.e., $u(t,x):=p(t,x-\Lambda_t)$, $x\ge\Lambda_t$, $t\in[0,T]$ is the solution of \eqref{eq:Stefan} in $W^{1,2}_2(\{(t,x)\in[0,T]\times[0,\infty):\,x\ge\Lambda_t\})$.

\medskip

Due to the absence of the derivative $\dot{\Lambda}$ in the probabilistic formulation \eqref{eq::init1}--\eqref{eq::init2}, the latter allows to study the liquid-solid boundary $\Lambda$ for all times. As noted in \cite[Theorem 1.1]{HLS}, $\Lambda$ cannot be continuous for all $t\in[0,\infty)$ when $\E[X_{0-}]<\frac{\alpha}{2}$, which necessitates to consider the solutions of \eqref{eq::init1}--\eqref{eq::init2} in the space $D([0,\infty))$ of right-continuous functions with left limits in general. However, in $D([0,\infty))$ uniqueness does not hold for \eqref{eq::init1}--\eqref{eq::init2}, since the jump sizes of $\Lambda$ are not determined uniquely by \eqref{eq::init1} and \eqref{eq::init2} alone (see, e.g., \cite[Example 2.2, Figure 3]{HLS}, \\ as well as \cite[p.~7, last paragraph]{NS2}, \cite[discussion preceding Definition 2.2]{DIRT}). %Nonetheless, there is a unique \textit{physical} solution of \eqref{eq::init1}--\eqref{eq::init2}, namely one with the property 
We will consider those solutions where the jump sizes are chosen as
\begin{equation}\label{physical}
	\Lambda_t-\Lambda_{t-}=\inf\Big\{x>0:\,\pp\big(\tau\ge t,\,X_{t-}\in(0,x]\big)<\frac{x}{\alpha}\Big\},\;\;t\ge 0, 
\end{equation} 
with $\Lambda_{t-}:=\lim_{s\uparrow t} \Lambda_s$ and $X_{t-}:=\lim_{s\uparrow t} X_s$. Physically, \eqref{physical} states that the supercooled liquid heats up to its equilibrium freezing temperature and freezes on the smallest interval $[\Lambda_{t-},\Lambda_{t-}+x)$ for which this transition is energy neutral. Similarly, when \eqref{eq::init1}--\eqref{eq::init2} and its variants arise in the large system limit of systemic risk models in finance (see \cite{NS1,HLS,LS}), or of integrate-and-fire models in neuroscience (see \cite{DIRT}), only the solutions with the minimality property \eqref{physical} seem economically, or biologically, relevant. Under the Assumption \ref{ass}(a), the solution $\Lambda$ of \eqref{eq::init1}--\eqref{eq::init2} in $D([0,\infty))$ satisfying \eqref{physical} is unique (see \cite[Theorem 1.4]{DNS}), and it is referred to as the \textit{physical solution} of \eqref{eq::init1}--\eqref{eq::init2}. 

\begin{ass}\label{ass}
\begin{enumerate}[(a)]
	\item $X_{0-}\!\!\ge\!0$ possesses a bounded density $f$ on $[0, \infty)$ that changes monotonicity finitely often on compacts.
	\item There exists a physical solution of \eqref{eq::init1}--\eqref{eq::init2} starting from $X_{0-}$. 
\end{enumerate}	
\end{ass}

\noindent The existence of a physical solution is shown for $X_{0-}\!\ge\!0$ with $\E[X_{0-}]\!<\!\infty$ in \cite[Theorem~6.5]{CRS}, building in part on \cite[proof of Theorem 3.2]{LS} which made stronger assumptions on $X_{0-}$ (see also \cite[Theorem 4.4]{DIRT2}, \cite[Theorem 2.3]{NS1} for existence results in related contexts). 

%This equation is a McKean-Vlasov problem, first occurring as a model of a large network of electrically coupled neurons, as well as a model for large financial networks with contagious default. Hambly, Ledger, and Sojmark proved that there exist choices of $\alpha$ and $Y_0$ such that this equation admits no continuous solutions, and that
%Hambly, Ledger, and Sojmark showed that {\color{blue} for sufficiently large $\alpha$, $L$ (and subsequently $Y$) is necessarily discontinuous, and}
%\eqref{eq::init1} and \eqref{eq::init2} admits a unique solution up to the first time where $L$ and $Y$ are discontinuous, provided that 
%the law of $Y_0$ has density bounded near the origin in the following sense:
%the density of $Y_0$ is 0 and H{\"o}lder continuous at 0.
%satisfies, for all $x$,
%\begin{eqnarray}
%\label{init_dens}
%\phi(x) \le B x^{\beta}
%\end{eqnarray}
%for some $B, \beta > 0$ independent of $x$. 
%They conjectured that uniqueness holds over all times if we consider only c\`{a}dl\`{a}g physical solutions. This conjecture was proven by Delarue, Nadtochiy, and Shkolnikov for a large range of initial conditions in \cite{DNS}, under the
%They then proceeded to consider c\`{a}dl\`{a}g solutions to the equation. They conjectured that with an additional constraint on the solution at points of discontinuity, the system would admit a unique solution given $\alpha$ and $Y_0$.
%constraint of a ``physical solution'', first introduced by Delarue, Inglis, Rubenthaler, and Taur\'{e} for a similar equation. \cite{HLS} \cite{DIRT}
%Before defining the notation of a physical solution, we first remark 
%We remark that any solution $(Y, L)$ to \eqref{eq::init1} and \eqref{eq::init2} can be solely defined by the deterministic variable $L$; from there, \eqref{eq::init1} would give us $Y$ in terms of $Y_0$. 

%In all the described applications, the absence of a closed-form solution makes it of great interest to find a numerical scheme allowing to accurately approximate the physical solution $\Lambda$ of \eqref{eq::init1}--\eqref{eq::init2} given any $f$ and $\alpha$. In \cite{KR}, the following general strategy has been proposed: 
%

\medskip

The absence of a closed-form solution calls for numerical methods. Proposed methods include approximations to Volterra equations that $\Lambda$ solves (see \cite{lipton2019semi}) and a fixed-point iteration in the space of boundaries (see \cite{CRS}). Herein, we follow the general strategy of \cite{KR}:
\begin{itemize}
	\item Define a discrete process $\widetilde{X}$ and a discrete function $\widetilde{\Lambda}$ such that $\widetilde{X}$ and $\widetilde{\Lambda}$ are close to $X$ and $\Lambda$ in some sense.
	\item Approximate $\widetilde{X}$ and $\widetilde{\Lambda}$ by a representative particle in a particle system $\{\overline{X}^i\}_{i=1}^N$ and a corresponding estimator $\overline{\Lambda}^N$, which can be generated through simulation.
\end{itemize}
Subsequently, given a discrete time step $\Delta>0$, the following natural definition of $(\widetilde{X},\widetilde{\Lambda})$, referred to as $(X^\Delta,\Lambda^\Delta)$, is chosen in \cite{KR}.   

\begin{dfn}\label{defn::discrete}
	Let $X^\Delta_{n\Delta}$, $n=0,\,1,\,\ldots$ and $\Lambda^\Delta_{n\Delta}$, $n=1,\,2,\,\ldots$ be defined recursively by $X^\Delta_0=X_0$, 
	\begin{equation}\label{eq::init_discrete}
		\Lambda^{\Delta}_{n\Delta}=\alpha\pp\Big(\min_{0\le m\le n-1} X^\Delta_{m\Delta}<0\Big),\;n=1,2,\ldots\;\text{and}\; X^\Delta_{n\Delta}=X_{0-}+B_{n\Delta}-\Lambda^\Delta_{n\Delta},\;n=1,2,\ldots.  
	\end{equation}
	We extrapolate by setting $\Lambda^\Delta_{0-}=0$, $\Lambda^\Delta_0=\alpha\pp(X_0\le0)$ and $\Lambda^{\Delta}_t=\Lambda^{\Delta}_{\lfloor t/\Delta \rfloor \Delta}$, $t>0$, as well as $X^\Delta_{0-}=X_{0-}$ and $X^{\Delta}_t = X_{0-} + B_t - \Lambda^{\Delta}_t$, $t\ge0$. 
\end{dfn}

It is shown in \cite[Theorem 1]{KR} that under the additional decay assumption $f(x)=O(x^\beta)$, $x\downarrow0$ for some $\beta\in(0,1]$ (originally introduced in \cite{HLS}) the convergence $\Lambda^\Delta\underset{\Delta\downarrow0}{\longrightarrow}\Lambda$ holds uniformly in time on a sufficiently small interval $[0,T]$, depending on the model parameters and preceding the first jump of $\Lambda$, with an order arbitrarily close to $\frac{1}{2}$. In the classical setting of stochastic differential equations (SDEs) with Lipschitz coefficients, the strong order of the Euler-Maruyama scheme, of which the above is a variant, is $\frac{1}{2}$, but increases to $1$ if the diffusion coefficient is constant (as is the case here) since the Euler scheme coincides with the first order Milstein scheme in this case. % (see, e.g., \textcolor{red}{reference}).

The reduction of the convergence rate in the present setting comes from (a) the possible non-Lipschitzianity of the densities of $X_t\,\mathbf{1}_{\{\tau>t\}}$ at $0$ and (hence) of the bounded variation part $-\Lambda$ of $X$, and (b) the underestimation of the hitting probability between time steps. In the setting of \cite{KR}, these difficulties can be resolved to obtain convergence of order $1$ in the following way (see \cite[Corollary 1]{KR}): refining the time mesh close to time $0$ where $\dot{\Lambda}$ has a singularity, and
%in the density of $X_t\,\mathbf{1}_{\{\tau>t\}}$ at $0$, 
using a continuous-time Brownian bridge interpolation of the Euler--Maruyama scheme as in \cite{gobet2000weak} to correct the leading order term in $\Delta$ of the hitting probability.
As the loss function with interpolation lies between the approximate loss function for our time-stepping scheme and the true loss function, the global convergence result below extends automatically to the scheme with interpolation. An improvement of the convergence order will only be observed locally where the loss function is sufficiently regular. The time mesh refinement in  \cite{KR} relies on explicit knowledge of the polynomial order of the singularity of $\dot{\Lambda}$ at $t=0$.
%More generally, starting from a continuity point with known initial condition, one may be able to use the modulus of continuity as given in Corollary \ref{cor:mod_of_cont} to control the local error by modifying the step size as a function of $t$ in the proof of Proposition \ref{prop:loc_conv}.
Although we give a modulus of right-continuity for $\Lambda$ in Corollary~\ref{cor:mod_of_cont}, it is unclear how it can be leveraged to control the local error by mesh refinement and obtain a higher convergence order. It may be possible to construct an adaptive scheme which estimates heuristically the local regularity of $\Lambda$, in particular in the run-up to a singularity, but this is beyond the scope of the present paper.

\medskip

Our main result is concerned with the convergence of $\Lambda^\Delta$ to $\Lambda$ \textit{globally} in time. For each $T\in(0,\infty)$, we let $D([0,T])$ be the space of real-valued functions on $[0,T]$ that are right-continuous at all $t\in[0,T)$ and have left limits at all $t\in(0,T]$. We endow $D([0,T])$ with the topology of Skorokhod M1 convergence from \cite{Sko}, whose definition for non-decreasing functions is recalled in Subsection \ref{subsec:M1} for the convenience of the reader. Our main result can then be stated as follows. 

\begin{thm}\label{thm::main}
Under Assumption \ref{ass} and for any continuity point $T\in(0,\infty)$ of $\Lambda$, it holds $\Lambda^\Delta|_{[0,T]}\overset{\emph{M1}}{\underset{\Delta\downarrow0}{\longrightarrow}}\Lambda|_{[0,T]}$ in $D([0,T])$.   
\end{thm}

\begin{rmk}
	The notion of convergence in Theorem \ref{thm::main} is often referred to as M1 convergence in $D([0,\infty))$, see, e.g., \cite[Section 12.9]{Whi}. In particular, for any $T\in(0,\infty)$ such that $\Lambda|_{[0,T]}$ is continuous, this notion of convergence yields the uniform convergence $\sup_{t\in[0,T]} |\Lambda^\Delta_t-\Lambda_t|\underset{\Delta\downarrow0}{\longrightarrow}0$ (use, e.g., \cite[Corollary 12.5.1, then implication (v)$\Rightarrow$(i) in Theorem 12.4.1, and finally Lemma 12.4.2]{Whi}). Thus, Theorem \ref{thm::main} naturally includes the convergences addressed in \cite[Theorems 1, 4]{KR}. Moreover, Theorem \ref{thm::main} gives the almost sure convergence of $X^\Delta=X_{0-}+B-\Lambda^\Delta$ to $X=X_{0-}+B-\Lambda$ with respect to the M1 convergence in $D([0,\infty))$, thanks to \cite[Corollary 12.7.1]{Whi}.
	
	%Assumption \ref{ass}(b) in Theorem \ref{thm::main} is only needed to guarantee the existence of a physical solution and can be swapped for any assumption ensuring the latter. 
\end{rmk}


A crucial and novel element of our analysis is the argument that for vanishing mesh size the numerical solution approaches the true physical solution immediately after a jump. This is achieved by first showing that the probability density of the numerical solution is arbitrarily close to that of the true physical solution immediately prior to the jump, and then using this property to prove that the numerical solution ``catches up'' arbitrarily fast with the physical solution after the jump of the latter (see Figure \ref{fig:example2} for an illustration). The convergence of the explicit Euler-type scheme to the \emph{physical} solution herein is akin to that of a system with delays to the physical solution in \cite[Theorem 4.9]{DIRT}. The physicality of the limit can be rationalized by noticing that the numerical approximations converge from below, and reveals that other than by a minimality property the physical solution is also characterized as the continuous-time limit of a discrete approximation with a delayed self-reinforcement effect. This differs from the proofs of \cite[Theorem~4.7]{DIRT}, \cite[Theorem 2.3]{NS1}, \cite[Theorem 3.2]{LS} which show the convergence of approximating particle systems to the physical solution. There, it is hard to rule out ``overshooting'' (non-physicality) of the limit.

\medskip

In the course of the proof of Theorem \ref{thm::main} we obtain an explicit bound on the rate of convergence \textit{locally} in time, which varies according to the density of $X_0$ on a right neighborhood of $0$. This result, interesting on its own, is reported in Theorem \ref{thm:loc_conv}. 

\begin{thm}\label{thm:loc_conv}
Suppose Assumption \ref{ass}. Let the density of $X_0$ be less or equal to $\frac{1}{\alpha}-\psi$ on an interval $(0,\delta]$, with a strictly increasing function $\psi:\,(0,\delta]\to(0,\infty)$. For $x\in(0,\delta]$, define $\Psi(x)\!=\!\int_0^x \psi(y)\,\mathrm{d}y$ and
\begin{equation}
\widetilde{\Psi}(x)=\Bigg\lbrace\!\!\begin{array}{ll} 
c_1x & \text{if}\;\;\psi(0):=\lim_{y\downarrow 0} \psi(y)>0, \\
c_2\int_0^x \Phi\big(q-\frac{c_3}{\Psi(y)}\big)\,\mathrm{d}y & \text{if}\;\;\psi(0)=0,
\end{array}
\end{equation}
where $\Phi$ is the standard Gaussian cumulative distribution function, 
 \begin{eqnarray}
 && c_1:=\frac{1}{4}\Big(\psi(0)-\big(2\|f\|_\infty+\psi(0)-1/\alpha\big)_+\,e^{-\frac{\delta^2}{3\teps}}\Big)>0, \qquad \\
&& c_2:=\psi(\delta/2)-\big(2\|f\|_\infty+\psi(\delta/2)-1/\alpha\big)_+\,e^{-\frac{7\delta^2}{24\teps}}>0, \qquad \\
&& c_3:=\big(\|f\|_\infty\,\sqrt{2/\pi}-q\psi(\delta)\big)\,\delta/2>0, \qquad \\
&& q:=\Phi^{-1}(1/4)<0, \qquad \\
&& 0<\teps<\begin{cases}
\min\Big(\frac{\pi}{8\|f\|_\infty^2}\,\Psi(\delta/6)^2,\,\frac{\delta^2}{3\log\max(1,(2\|f\|_\infty+\psi(0)-1/\alpha)_+/\psi(0))}\Big) & \text{if}\;\;\psi(0)\!>\!0, \\
\frac{\pi}{8\|f\|_\infty^2}\,\Psi(\delta/6)^2 & \text{if}\;\;\psi(0)\!=\!0.
\end{cases} \label{teps:UBD} \qquad
\end{eqnarray} 	
Then, for all $\teps$ adhering to \eqref{teps:UBD} and all $\Delta>0$ small enough,
\begin{eqnarray}
\sup_{s\in[0,\teps]} |\Lambda^\Delta_s\!-\!\Lambda_s| \le
\widetilde{\Psi}^{-1}\Big(\|f\|_\infty\Big(\!192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
\!+\!2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big)\!\Big) \qquad\; && \label{roc} \\
+\max(\alpha\|f\|_\infty,1)\Big(\!192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
\!+\!2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big). && \nonumber
\end{eqnarray}
\end{thm}

\begin{rmk}
Assumption \ref{ass}(a) and the condition \eqref{physical} together imply that the density of $X_0$ is necessarily less or equal to $\frac{1}{\alpha}-\psi$ on an interval $(0,\delta]$, for some strictly increasing function $\psi:\,(0,\delta]\to(0,\infty)$. If the density of $X_0$ is such that $\delta>0$ can be chosen arbitrarily large, then the upper bound on $\teps$ in \eqref{teps:UBD} can be made arbitrarily large, rendering \eqref{roc} a \textit{global} estimate. In general, however, to control the rate of convergence globally one needs a quantitative bound on the density of $X_t\,\mathbf{1}_{\{\tau>t\}}$ on a right neighborhood of $0$ for an arbitrary $t\ge0$, which has proved elusive. 
\end{rmk}

\begin{rmk}
\label{rm_order}
		\!\!(a) When $\psi(0)\!>0$, we may swap $\psi$ for the constant $\psi(0)$, simplifying \eqref{roc} to 
			\begin{equation}\label{roc_simplified}
			\sup_{s\in[0,\teps]} |\Lambda^\Delta_s-\Lambda_s| \le
			c_4\sqrt{\Delta}\,\big(\sqrt{\log(\lceil\teps/\Delta\rceil/2)}+c_5\big)
			\end{equation}
		and \eqref{teps:UBD} to $0<\teps<c_6\delta^2$, with 
		$c_4:=192\sqrt{2}\,\big(\|f\|_\infty/c_1+\max(\alpha\|f\|_\infty,1)\big)$, 
		$c_5:=\frac{\|f\|_\infty}{48\sqrt{2\pi}\psi(0)}$, and 
		%$c_5:=\|f\|_\infty/(48\sqrt{2\pi}\psi(0))$, and 
		$c_6:=\min\big(\frac{\pi\psi(0)^2}{288\|f\|_\infty^2},\,\frac{1}{3\log\max(1,(2\|f\|_\infty+\psi(0)-1/\alpha)_+/\psi(0))}\big)$. 
		As we detail in Subsection \ref{sim1/2}, the theoretical order $\frac{1}{2}$ in \eqref{roc_simplified} agrees with the one found in numerical simulations. 
		
		\vspace{5pt}
		
		\noindent (b) When $\psi(0)=0$, we have $\lim_{x\downarrow0} \widetilde{\Psi}^{-1}(x)=0$ and $\lim_{x\downarrow0} (\widetilde{\Psi}^{-1})'(x)=\infty$, so that the $\widetilde{\Psi}^{-1}$-term on the right-hand side of \eqref{roc} determines its order of magnitude in $\Delta$. As we illustrate in 
		Subsection \ref{sec5.3}, the order observed in numerical simulations agrees instead with that of the term on the second line in \eqref{roc}. This leads us to conjecture that, in fact, the latter gives the true order of the left-hand side of \eqref{roc} in $\Delta$, whereas the $\widetilde{\Psi}^{-1}$-term on the right-hand side of \eqref{roc} is an artifact of our proof technique. Specifically, if $\partial_x^b \psi(0+) = 0$, $b=0,\,1,\,\ldots,\,a-1$, $\partial_x^a \psi(0+) > 0$, as for the monomials $x^a$ in Subsection \ref{sec5.3},
it would yield the order $1/(2(a+1))$ noticed in the numerical experiments. For $\psi$ with vanishing derivatives at $0$ of all orders, we do not expect to see a positive covergence order, but it is hard to check this claim numerically.
\end{rmk}

The rest of the paper is structured as follows. In Section \ref{sec:prelim}, we collect a number of preliminaries: a classification of time points for the physical solution (Subsection \ref{classi}); explicit estimates on the densities of $X_s\,\mathbf{1}_{\{\tau>s\}}$ and $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ near $0$, as well as on the increments of $\Lambda$, in right time neighborhoods (Subsection \ref{rightn}); and definitions of the Skorokhod M1 convergence for non-decreasing functions and of some auxiliary time-stepping schemes (Subsection \ref{subsec:M1}). In Section \ref{sec:loc_conv}, we prove Theorem \ref{thm:loc_conv} by an inductive argument relying on the results of Subsection \ref{rightn}. Subsequently, in Section \ref{sec:mainproof}, we show our main result (Theorem \ref{thm::main}) by extending Theorem \ref{thm:loc_conv} to the statement that the M1 convergence $\Lambda^\Delta\underset{\Delta\downarrow0}{\longrightarrow}\Lambda$ on an interval $[0,T)$ implies the M1 convergence $\Lambda^\Delta|_{[0,T+\teps]}\underset{\Delta\downarrow0}{\longrightarrow}\Lambda|_{[0,T+\teps]}$ for some $\teps>0$. We achieve this separately for the cases that $T$ is a continuity point of $\Lambda$ (Subsection~\ref{sec::no_jump}) and that $T$ is a discontinuity point of $\Lambda$ (Subsection \ref{sec::special_case}). In both cases, we build on Theorem \ref{thm:loc_conv} and the error propagation bounds of Subsection \ref{sec::stab}. Subsection \ref{sec::post_jump} then offers the main line of the proof of Theorem \ref{thm::main}. In Section \ref{sec::numerical}, we give the results of our simulations, based on a particle approximation, and compare them with the theoretical findings. The convergence rate of this particle approximation is controlled in the appendix.

\medskip

\noindent\textbf{Acknowledgement.} M.~Shkolnikov has been partially supported by the NSF grants DMS-1811723, DMS-2108680 and a Princeton SEAS innovation research grant. 

 


==> arXiv v2/Section2,5_new.tex <==
%!TEX root =Main.tex

\section{Proof of Theorem \ref{thm:loc_conv}} \label{sec:loc_conv}

In this section, we establish the following generalization of Theorem \ref{thm:loc_conv} to arbitrary $t\ge0$ (instead of only $t=0$), which is also used in the proof of Theorem \ref{thm::main} below. 

\begin{prop}\label{prop:loc_conv}
In the situation of Proposition \ref{prop:density_est}, let $\frac{1}{\alpha}-\widetilde{\psi}:\,(-\delta,0)\to\big[0,\frac{1}{\alpha}\big)$ be the function in \eqref{<0UBD} and $\widetilde{\Psi}(x):=\int_0^x \widetilde{\psi}(-y)\,\mathrm{d}y$, $x\in(0,\delta)$. Then, it holds 
\begin{equation}\label{loc_rate_conv}
\begin{split}
\sup_{s\in[t,t+\teps]} |\Lambda^{t;\Delta}_s-\Lambda_s| \le \widetilde{\Psi}^{-1}\Big(\|f\|_\infty\Big(192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
+2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big)\!\Big)\quad\;\;\; \\
+\max(\alpha\|f\|_\infty,1)\Big(192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
\!+\!2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big)
\end{split} 
\end{equation}
for all $\teps\!>\!0$ adhering to \eqref{teps:UBD} and all $\Delta>0$ small enough.
\end{prop}

\begin{rmk}
For a discontinuity point $t>0$, the function $\psi$ in Proposition \ref{prop:density_est} can be chosen as $cx^a$ for some $a\in{\mathbb N}$ and $c>0$ (see, e.g., \cite[proof of Theorem 3.3]{LS2}). Then, the argument of $\widetilde{\Psi}^{-1}$ and the term on the second line in \eqref{loc_rate_conv} have the order $1/(2(a+1))$ in $\Delta$. As touched upon in Remark \ref{rm_order}, we conjecture this to reflect the true order of the left-hand side in~\eqref{loc_rate_conv}, based on the numerical simulations described in Subsection \ref{sec5.3}.
\end{rmk}

\noindent\textbf{Proof of Proposition \ref{prop:loc_conv}.} Clearly, it suffices to check that each of $\Lambda_{t+n\Delta}-\Lambda^{t;\Delta}_{(t+n\Delta)-}$, $n=1,2,\ldots,\lceil\teps/\Delta\rceil$ does not exceed the right-hand side of \eqref{loc_rate_conv}. To this end, we argue by induction over $n$. For $n=1$, the result follows from $\Lambda^{t;\Delta}_{(t+\Delta)-}=\Lambda_t$ and Corollary \ref{cor:mod_of_cont}, so we turn to $n\ge 2$. We then have
\begin{equation}\label{eq:2diff}
\begin{split}
\Lambda_{t+n\Delta}\!-\!\Lambda^{t;\Delta}_{(t+n\Delta)-}&=\alpha\pp\Big(\inf_{0\le s\le t+n\Delta} X_s\le 0\Big)
\!-\!\alpha\pp\Big(\inf_{0\le s\le t} X_s\le 0\;\,\text{or}\;\min_{0\le m\le n-2} X^{t;\Delta}_{t+m\Delta}<0\Big) \\
&=\alpha\pp\Big(\tau>t,\,\inf_{t<s\le t+n\Delta} X_s\le 0\Big)
-\alpha\pp\Big(\tau>t,\,\min_{0\le m\le n-2} X^{t;\Delta}_{t+m\Delta}<0\Big) \\
& =\alpha\pp\Big(\tau>t,\,\inf_{t<s\le t+n\Delta} X_s\le 0\Big)
-\alpha\pp\Big(\tau>t,\,\min_{0\le m\le n-2} X_{t+m\Delta}<0\Big) \\
&\quad+\alpha\pp\Big(\tau\!>\!t,\,\min_{0\le m\le n-2} X_{t+m\Delta}<0\Big)
\!-\!\alpha\pp\Big(\tau\!>\!t,\,\min_{0\le m\le n-2} X^{t;\Delta}_{t+m\Delta}<0\Big).
\end{split}
\end{equation}

\smallskip

The difference on the third line in \eqref{eq:2diff} is bounded above by
\begin{equation*}
\begin{split}
& \;\alpha\pp\Big(0<X_t\,\mathbf{1}_{\{\tau>t\}}+\min_{0\le m\le n-2} (B_{t+m\Delta}-B_t-\Lambda_{t+m\Delta}+\Lambda_t) \\
&\qquad\;\;\,\le\sup_{{t\le s_1<s_2\le t+n\Delta}\atop{s_2-s_1\le 2\Delta}} |B_{s_2}-B_{s_1}|+\sup_{{t\le s_1<s_2\le t+n\Delta}\atop{s_2-s_1\le 2\Delta}} (\Lambda_{s_2}-\Lambda_{s_1})\!\Big) \\
& \le \alpha\|f\|_\infty\bigg(\E\Big[\sup_{{t\le s_1<s_2\le t+n\Delta}\atop{s_2-s_1\le 2\Delta}} |B_{s_2}-B_{s_1}|\Big]+\sup_{{t\le s_1<s_2\le t+n\Delta}\atop{s_2-s_1\le 2\Delta}} (\Lambda_{s_2}-\Lambda_{s_1})\!\bigg) \\
& \le \alpha\|f\|_\infty\Big(192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
+2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big), 
\end{split}
\end{equation*}
where we have used  \cite[Lemma 4 and Remark 3]{Fi} and Corollary \ref{cor:mod_of_cont}. The difference on the fourth line in \eqref{eq:2diff} can be estimated by 
\begin{equation*}
\begin{split}
&\;\alpha\pp\Big(-\max_{0\le m\le n-2}\,\big(\Lambda_{t+m\Delta}-\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)\le\min_{0\le m\le n-2} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}<0\Big) \\
&\le \max_{0\le m\le n-2}\,\big(\Lambda_{t+m\Delta}-\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)
-\alpha\widetilde{\Psi}\Big(\max_{0\le m\le n-2}\big(\Lambda_{t+m\Delta}-\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)\!\Big)
\end{split}
\end{equation*}
thanks to the induction hypothesis and Proposition \ref{prop:density_est}(b). 

\medskip

All in all, we have obtained
\begin{equation*}
\begin{split}
\Lambda_{t+n\Delta}\!-\!\Lambda^{t;\Delta}_{(t+n\Delta)-}\le  & \,\max_{0\le m\le n-2} \big(\Lambda_{t+m\Delta}\!-\!\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)
-\alpha\widetilde{\Psi}\Big(\max_{0\le m\le n-2}\big(\Lambda_{t+m\Delta}\!-\!\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)\!\Big) \\
&+\alpha\|f\|_\infty\Big(192\sqrt{2\Delta\log(\lceil\teps/\Delta\rceil/2)} 
+2\Psi^{-1}\big(2\sqrt{\pi}^{-1}\|f\|_\infty\sqrt{\Delta}\big)\!\Big).
\end{split}
\end{equation*}
We conclude by distinguishing the cases of how $\max_{0\le m\le n-2}\big(\Lambda_{t+m\Delta}-\Lambda^{t;\Delta}_{(t+m\Delta)-}\big)$ compares to the $\widetilde{\Psi}^{-1}$-term in \eqref{loc_rate_conv} and using the induction hypothesis. \qed  

\begin{rmk}\label{alt_ass}
It is worth noting that the proof of Proposition \ref{prop:loc_conv} (and thus, of Theorem~\ref{thm:loc_conv}) remains intact if instead of Assumption \ref{ass}(a), the boundedness of $f$ on $[0,\infty)$ together with the conclusions of Lemma \ref{lemma:a priori} and Corollary~\ref{cor:mod_of_cont} are assumed and $\psi:=\Psi':\,(0,\delta]\to\big(0,\frac{1}{\alpha}\big]$ is a strictly increasing function. Indeed, the proofs of Propositions \ref{prop:loc_conv} and \ref{prop:density_est}(b) can be then repeated word by word. 
\end{rmk}


==> arXiv v2/Section2_new.tex <==
%!TEX root =Main.tex

\section{Preliminaries} \label{sec:prelim}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Classification of time points}\label{classi}
%%%%%%%%%%%%%%%%%%%%%%%%

The basis of our analysis is the following proposition (see \cite[Theorem 1.4, first statement of Theorem 1.1]{DNS} and recall the minimality property~\eqref{physical}).
%The following definition prescribes the times at which $\Lambda$ (and hence $X$) is continuous, and the size of the discontinuity when it is discontinuous.
%\begin{definition}\label{defn::physical}
%	We call a solution $(X, \Lambda)$ to a \emph{physical solution} if 
%	\[
%		\Lambda_t-\Lambda_{t-}=\inf\Big\{x>0:\,\pp\big(\tau\ge t,\,X_{t-}\in(0,x]\big)<\frac{x}{\alpha}\Big\},\;\;t\ge 0, 
%	L_{t} - \lim_{s \to t^-} L_s = \frac{1}{\alpha}\left\{ \inf_{x} \left(\BPP(Y_{t^-} < x, \inf_{s < t} Y_{s} > 0) < \frac{1}{\alpha} x\right) \right\},
%	\]
%	for all times $t$.
%\end{definition}
%Moreover, each $t\ge $ falls into exactly one of the following categories:
%\begin{eqnarray}
%\mathbb{T}^{\rm (i)} &:=& \big\{t\ge 0 \,: \, \limsup_{x\downarrow0} x^{-1}\rho(t,x)<\infty \big\}, \\
%\mathbb{T}^{\rm (ii)} &:=& \big\{t\ge 0 \,: \, \limsup_{x\downarrow0} x^{-1}\rho(t,x)=\infty \text{ but } \lim_{x\downarrow0} \rho(t,x)<\frac{1}{\alpha} \big\}, \\
%\mathbb{T}^{\rm (iii)} &:=& \big\{t\ge 0 \,: \, \lim_{x\downarrow0} \rho(t,x)\ge\frac{1}{\alpha} \big\}.
%\end{eqnarray}
%For future reference, we define by $\mathbb{T}^{\rm (i)}$,  $\mathbb{T}^{\rm (ii)}$, and  $\mathbb{T}^{\rm (iii)}$, the sets of all times $t$ for which properties (i), (ii), and (iii) hold,	respectively. 
%Furthermore, we have the following characterisation of the regularity of the solution.
\begin{prop}\label{thm1}
Suppose Assumption \ref{ass}. Then, the physical solution is unique, and each $t\ge0$ falls into exactly one of the two categories: 
\begin{enumerate}[(i)]
\item For some $\delta>0$ and a strictly increasing function $\psi:\,(0,\delta]\to(0,\infty)$, the density of $X_{t-}\,\mathbf{1}_{\{\tau\ge t\}}$ on $(0,\delta]$ is bounded above by $\frac{1}{\alpha}-\psi$. In particular, $\Lambda_t=\Lambda_{t-}$.  
\item For some $\delta>0$ and a non-decreasing function $\psi:(0,\delta]\to[0,\infty)$, the density of $X_{t-}\,\mathbf{1}_{\{\tau\ge t\}}$ on $(0,\delta]$ is bounded below by $\frac{1}{\alpha}+\psi$. In particular, $\Lambda_t>\Lambda_{t-}$, and the density of $X_t\,\mathbf{1}_{\{\tau>t\}}=(X_{t-}-(\Lambda_t-\Lambda_{t-}))\,\mathbf{1}_{\{\tau>t\}}$ on $(0,\widetilde{\delta}]$ is bounded above by $\frac{1}{\alpha}-\widetilde{\psi}$, for some $\widetilde{\delta}>0$ and a strictly increasing function $\widetilde{\psi}:\,(0,\widetilde{\delta}]\to(0,\infty)$. 
\end{enumerate}
 \end{prop}

We refer to $t\ge0$ of categories (i) and (ii) in Proposition \ref{thm1} simply as \textit{continuity} and \textit{discontinuity points}.  

%\textcolor{red}{With the discrete approximation $(X^\Delta, \Lambda^\Delta)$ to $(X, \Lambda)$ from Definition 1, convergence has been shown under restrictive regularity assumptions on the initial value and for small enough times not exceeding the time of the first discontinuity.}
%\textcolor{red}{\begin{theorem}[Theorem 1 in \cite{KR}]\label{thm::kr}
%Assume there are $\overline{B}, \beta >0$ such that $f$ satisfies
%\begin{eqnarray}
%\label{init_dens}
%f(x) \le \overline{B} x^{\beta}
%\end{eqnarray}
%for all $x\ge 0$, and there is $\hat{B}>0$ such that
%\begin{eqnarray}\label{L_prime}
%\dot{\Lambda}_t \le \hat{B} \, t^{-\frac{1-\beta}{2}}
%\end{eqnarray}
%for all $t \in (0,T]$. Assume further that $T$ is small enough that
%\begin{eqnarray}\label{cond_T}
%\alpha \overline{B} \left[\sqrt{\frac{2T}{\pi}} + \frac{2\alpha\hat{B}}{1+\beta}T^{\frac{1+\beta}{2}} \right] < 1.
%\end{eqnarray}
%Then $\Lambda^\Delta \rightarrow \Lambda$ uniformly  on $[0, T]$ for $\Delta \rightarrow 0$. Furthermore, for every $p < 1/2$ there is a constant $C_{p}>0$ such that for all $t \in [0,T]$
%\[
%0 \le \Lambda_t - \Lambda^\Delta_t  \le C_p \Delta^p.
%\]
%\end{theorem}}

%\textcolor{red}{\begin{remark}
%It follows from \cite[Theorem 1.8]{HLS} that
%(\ref{init_dens}) implies (\ref{L_prime}) almost everywhere in a small enough time interval.
%\end{remark}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Regularity estimates in right time neighborhoods} \label{rightn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this subsection, we consider an arbitrary $t\ge0$ and provide explicit estimates on the densities of $X_s\,\mathbf{1}_{\{\tau>s\}}$, $s\in(t,t+\teps]$ and $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$, $n=0,1,\ldots,\lfloor\teps/\Delta\rfloor$ in the vicinity of $0$, for suitable (explicit) $\teps>0$. These estimates play a crucial role in our proof of Theorem \ref{thm:loc_conv}.  

\begin{prop}\label{prop:density_est}
Suppose Assumption \ref{ass}. Let $t\ge0$ be a continuity (discontinuity resp.) point, with the density of $X_{t-}\,\mathbf{1}_{\{\tau\ge t\}}$ ($X_t\,\mathbf{1}_{\{\tau>t\}}$ resp.) on an interval $(0,\delta]$ being bounded above by $\frac{1}{\alpha}-\psi$ for a strictly increasing function $\psi:\,(0,\delta]\to(0,\infty)$. Then, with $\Psi(x):=\int_0^x \psi(y)\,\mathrm{d}y$, $x\in(0,\delta]$:
\begin{enumerate}[(a)]
	\item The density of $X_s\,\mathbf{1}_{\{\tau>s\}}$ on $(0,\delta/6)$ cannot exceed $\frac{1}{\alpha}-\frac{\psi}{2}$ for any 
	\begin{equation}
	t<s<t+\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta/6)^2.
	\end{equation} 
	\item The density of $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ on $(-\delta,0)$ is bounded above by
    \begin{equation}\label{<0UBD}
    \begin{cases}
    \frac{1}{\alpha}-c_1 & \text{if}\;\;\;\psi(0):=\lim_{y\downarrow 0} \psi(y)>0, \\
    \frac{1}{\alpha}-c_2\,\Phi\big(q-\frac{c_3}{\Psi(-x)}\big) & \text{if}\;\;\;\psi(0)=0,
    \end{cases}
    \end{equation}	
    $n=1,2,\ldots,\lfloor\teps/\Delta\rfloor$, $\Delta>0$, where $\Phi$, $c_1$, $c_2$, $c_3$, $q$ and $\teps$ are as in Theorem \ref{thm:loc_conv}. 
   %is the standard Gaussian cumulative distribution function, 
   %\begin{eqnarray}
   %&& \teps<\begin{cases}
   %\min\Big(\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta/6)^2,\,\frac{\delta^2}{3\log\max(1,(4\|f\|_\infty+\psi(0)-1/\alpha)_+/\psi(0))}\Big) & \text{if}\;\;\psi(0)>0, \\
   %\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta/6)^2 & \text{if}\;\;\psi(0)=0,
   %\end{cases} \\
    %&& c_1:=\frac{1}{4}\Big(\psi(0)-\big(4\|f\|_\infty+\psi(0)-1/\alpha\big)_+\,e^{-\frac{\delta^2}{3\teps}}\Big)>0, \\
    %&& c_2:=\psi(\delta/2)-\big(2\|f\|_\infty+\psi(\delta/2)-1/\alpha\big)_+\,e^{-\frac{7\delta^2}{24\teps}}>0, \\
    %&& c_3:=\big(\|f\|_\infty\,\sqrt{2/\pi}-q\psi(\delta)\big)\,\delta/2>0, \\
    %&& q:=\inf\{y\in\rr:\,\Phi(y)=1/4\}<0.
    %\end{eqnarray} 	
\end{enumerate}
\end{prop}

Our~proof~of~Proposition~\ref{prop:density_est}~relies~on~an~(explicit)~\textit{a}~\textit{priori}~estimate~on~the~increments~of~$\Lambda$. 

\begin{lem}\label{lemma:a priori}
In the situation of Proposition \ref{prop:density_est}, we have
\begin{equation}
\Lambda_s-\Lambda_t \le \Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{s-t}\big),
\end{equation}
for all 
\begin{equation}\label{s_def}
t<s<\min\bigg(t+\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta)^2,\,\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\}\!\bigg).
\end{equation} 
\end{lem}

\noindent\textbf{Proof.} We use the definition of $\Lambda$ in \eqref{eq::init2}, its monotonicity, and the bounds $\frac{1}{\alpha}-\psi$, $\|f\|_\infty$ on the density of $X_t\,\mathbf{1}_{\{\tau>t\}}$ on $(0,\delta]$, $(0,\infty)$, respectively, to obtain
\begin{equation*}
\begin{split}
&\;\Lambda_s-\Lambda_t = \alpha\pp\Big(\tau>t,\,\inf_{r\in(t,s]} \big(X_t+(B_r-B_t)-(\Lambda_r-\Lambda_t)\big) \le 0\Big) \\
& \le \alpha\pp\Big(\tau>t,\,\inf_{r\in(t,s]} \big(X_t+(B_r-B_t)-(\Lambda_s-\Lambda_t)\big) \le 0\Big) \\
& \le \alpha\int_0^{\Lambda_s-\Lambda_t} \left(\frac{1}{\alpha}-\psi(x)\right)\,\mathrm{d}x+\alpha\int_{\Lambda_s-\Lambda_t}^\infty \|f\|_\infty\,\pp\Big(x+\inf_{r\in(t,s]} (B_r-B_t)-(\Lambda_s-\Lambda_t)\le 0\Big)\,\mathrm{d}x \\
&=\Lambda_s-\Lambda_t - \alpha\Psi(\Lambda_s-\Lambda_t)
+\alpha\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{s-t},
\end{split}
\end{equation*}
as long as $\Lambda_s-\Lambda_t<\delta$. In other words, $\Lambda_s-\Lambda_t<\delta$ implies
\begin{equation}
\Lambda_s-\Lambda_t\le\Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{s-t}\big). 
\end{equation}
The lemma readily follows upon noting that \eqref{s_def} enforces $\Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{s-t}\big)<\delta$. \qed

\medskip

We are now ready to give the proof of Proposition \ref{prop:density_est}. 

\medskip

\noindent\textbf{Proof of Proposition \ref{prop:density_est}. (a).} The density of $X_s\,\mathbf{1}_{\{\tau>s\}}$ on $(0,\infty)$ is bounded above by that of $\big(X_t+(B_s-B_t)-(\Lambda_s-\Lambda_t)\big)\,\mathbf{1}_{\{\tau>t\}}$. Recalling the notation $p(t,\cdot)$ for the density of $X_t\,\mathbf{1}_{\{\tau>t\}}$ on $(0,\infty)$ and writing $\varphi_{s-t}$ for the Gaussian density of mean $0$ and variance $s-t$, we can estimate the density of $\big(X_t+(B_s-B_t)-(\Lambda_s-\Lambda_t)\big)\,\mathbf{1}_{\{\tau>t\}}$ on $(0,\delta/6)$ by
\begin{equation*}
\begin{split}
&\,\int_{-\infty}^{-\frac{2}{3}\delta} p(t,x-y+\Lambda_s-\Lambda_t)\,\varphi_{s-t}(y)\,\mathrm{d}y
+\int_{-\frac{2}{3}\delta}^{x+\Lambda_s-\Lambda_t} p(t,x-y+\Lambda_s-\Lambda_t)\,\varphi_{s-t}(y)\,\mathrm{d}y \\
&\le\,\|f\|_\infty\,\Phi\bigg(\!-\frac{2\delta}{3\sqrt{s-t}}\bigg)
+\int_{-\frac{2}{3}\delta}^0 \bigg(\frac{1}{\alpha}-\psi(x-y+\Lambda_s-\Lambda_t)\!\bigg)\,\varphi_{s-t}(y)\,\mathrm{d}y \\
&\quad\;+\int_0^{x+\Lambda_s-\Lambda_t} \bigg(\frac{1}{\alpha}-\psi(x-y+\Lambda_s-\Lambda_t)\!\bigg)\,\varphi_{s-t}(y)\,\mathrm{d}y \\
&\le \,\|f\|_\infty\,\Phi\bigg(\!-\frac{2\delta}{3\sqrt{s-t}}\bigg)+\frac{1}{2}\,\bigg(\frac{1}{\alpha}-\psi(x)\!\bigg)
+\frac{1}{\alpha}\,\bigg(\frac{1}{2}-\Phi\bigg(\!-\frac{x+\Lambda_s-\Lambda_t}{\sqrt{s-t}}\bigg)\!\bigg),
\end{split}
\end{equation*}
provided that $\Lambda_s-\Lambda_t\le\delta/6$ (since then $x-y+\Lambda_s-\Lambda_t\in(0,\delta]$ for all $-\frac{2}{3}\delta\le y<x+\Lambda_s-\Lambda_t$) and where $\Phi$ is the standard Gaussian cumulative distribution function. Using $x\in(0,\delta/6)$ and the assumption $\Lambda_s-\Lambda_t\le\delta/6$ again we obtain the further upper bound 
\begin{equation*}
\frac{1}{\alpha}-\frac{\psi(x)}{2}
+\,\|f\|_\infty\,\Phi\bigg(\!-\frac{2\delta}{3\sqrt{s-t}}\bigg)-\frac{1}{\alpha}\,\Phi\bigg(\!-\frac{\delta}{3\sqrt{s-t}}\bigg).
\end{equation*} 
In view of the elementary inequality $\Phi(-2y)\le e^{-3y^2/2}\,\Phi(-y)$, $y>0$, it holds 
\begin{equation*}
\begin{split}
\frac{1}{\alpha}-\frac{\psi(x)}{2}
+\,\|f\|_\infty\,\Phi\bigg(\!-\frac{2\delta}{3\sqrt{s-t}}\bigg)-\frac{1}{\alpha}\,\Phi\bigg(\!-\frac{\delta}{3\sqrt{s-t}}\bigg)\le \frac{1}{\alpha}-\frac{\psi(x)}{2},\\ 
t<s<t+\frac{\delta^2}{6\log\max(\alpha\|f\|_\infty,1)}.
\end{split}
\end{equation*} 

\smallskip

Since $\Lambda_s-\Lambda_t\le\delta/6$ for all 
\begin{equation*}
t<s<\min\bigg(t+\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta/6)^2,\,\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\}\!\bigg)
\end{equation*}
by Lemma \ref{lemma:a priori}, we obtain the desired density estimate for all 
\begin{equation}\label{min3terms}
t<s<\min\bigg(t+\frac{\pi}{2\|f\|_\infty^2}\,\Psi(\delta/6)^2,\,\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\},\,t+\frac{\delta^2}{6\log\max(\alpha\|f\|_\infty,1)}\bigg).
\end{equation}
In view of $\psi\le\frac{1}{\alpha}$, one has $\Psi(\delta/6)\le\delta/(6\alpha)$, and we conclude by elementary calculations that the first term in the minimum is less or equal to the third term. It remains to show that $\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\}$ cannot attain the minimum in \eqref{min3terms}. Assuming the opposite and letting $\widetilde{t}:=\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\}<\infty$ we infer that the density of $X_{\widetilde{t}-}\,\mathbf{1}_{\{\tau\ge\widetilde{t}\}}=\lim_{r\uparrow\widetilde{t}} X_r\,\mathbf{1}_{\{\tau>r\}}$ on $(0,\delta/6)$ is bounded above by $\frac{1}{\alpha}-\frac{\psi}{2}$, thus $\Lambda_{\widetilde{t}}=\Lambda_{\widetilde{t}-}$ due to the minimality property \eqref{physical}. This and the right-continuity of $\Lambda$ at $\widetilde{t}$ contradict $\widetilde{t}=\inf\{r\!>\!t:\Lambda_r\!>\!\Lambda_{r-}\}<\infty$. 

\medskip

\noindent\textbf{(b).} Fix $\Delta>0$, $1\le n\le\lfloor\teps/\Delta\rfloor$ and denote the law of $\min_{0\le m\le n} (B_{t+m\Delta}-B_t-\Lambda_{t+m\Delta}+\Lambda_t)$ by $\mu$. The density of $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ on $(-\delta,0)$ is $\int_{(-\infty,x)} p(t,x-y)\,\mu(\mathrm{d}y)$, which can be bounded above by 
\begin{equation}\label{quantity}
\int_{(x-\delta,x)} \left(\frac{1}{\alpha}-\psi(x-y)\right)\,\mu(\mathrm{d}y) + \|f\|_\infty\,\mu\big((-\infty,x-\delta]\big).
\end{equation}
Next, we observe the inequalities 
\begin{equation}\label{ineq:comp}
\begin{split}
B_{t+n\Delta}-B_t-\Lambda_{t+n\Delta}+\Lambda_t &\ge\min_{0\le m\le n} (B_{t+m\Delta}-B_t-\Lambda_{t+m\Delta}+\Lambda_t) \\
&\ge \min_{t\le s\le t+n\Delta} (B_s-B_t) - (\Lambda_{t+n\Delta}-\Lambda_t)
\end{split}
\end{equation}
and introduce the notations $\widetilde{\varphi}$ and $\widetilde{\Phi}$ for the Gaussian density and cumulative distribution function of mean $-\Lambda_{t+n\Delta}+\Lambda_t$ and variance $n\Delta$. At this point, we distinguish two cases: $\mu\big((-\infty,x]\big)<\frac{1}{2}$ and $\mu\big((-\infty,x]\big)\ge\frac{1}{2}$. 

\medskip

In the first case, we apply $\mu\big((-\infty,x]\big)<\frac{1}{2}$, the second inequality in \eqref{ineq:comp} and the reflection principle for Brownian motion to estimate the density of $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ on $(-\delta,0)$ further by 
\begin{equation*}
\frac{1}{2\alpha}+2\|f\|_\infty\,\widetilde{\Phi}(x-\delta)
=\frac{1}{2\alpha}+2\|f\|_\infty\,\Phi\bigg(\frac{x-\delta+\Lambda_{t+n\Delta}-\Lambda_t}{\sqrt{n\Delta}}\bigg).
\end{equation*}
Since $x\le0$ and $\Lambda_{t+n\Delta}-\Lambda_t\le\delta/6$ (see the last paragraph in the proof of part (a)), the latter estimate is less or equal to $\frac{1}{2\alpha}+2\|f\|_\infty\,\Phi\big(\!-\frac{5\delta}{6\sqrt{\teps}}\big)$. An elementary calculation shows that the range of $\teps>0$ for which this is less than $\frac{1}{\alpha}$ contains the interval specified by \eqref{teps:UBD}. 

\medskip

In the second case, we upper bound the quantity in \eqref{quantity} by
\begin{equation*}
\int_{\rr} \Big( \frac{1}{\alpha}-\psi(x-y)\Big)\,\mathbf{1}_{(x-\delta,x)}(y)+\frac{1}{\alpha}\,\mathbf{1}_{[x,\infty)}(y)\,\mu(\mathrm{d}y)+\|f\|_\infty\,\mu\big((-\infty,x-\delta]\big).
\end{equation*}
Using the inequalities in \eqref{ineq:comp} and the reflection principle for Brownian motion, we estimate the density of $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ on $(-\delta,0)$ further by
\begin{equation}\label{expr}
\int_{\rr} \bigg(\!\Big( \frac{1}{\alpha}-\psi(x-y)\Big)\,\mathbf{1}_{(x-\delta,x)}(y)+\frac{1}{\alpha}\,\mathbf{1}_{[x,\infty)}(y)\!\bigg)
\,\widetilde{\varphi}(y)\,\mathrm{d}y +2\|f\|_\infty\,\widetilde{\Phi}(x-\delta).
\end{equation}
Next, we exploit that for any $z\in[0,\delta)$, it holds $\psi(x-y)\ge\psi(z)$, $y\in(x-\delta,x-z)$ and $\psi(x-y)\ge0$, $y\in[x-z,x)$. This allows to upper bound the expression in \eqref{expr} by
\begin{equation*}
\begin{split}
& \;\frac{1}{\alpha}\big(1-\widetilde{\Phi}(x-\delta)\big)-\psi(z)\big(\widetilde{\Phi}(x-z)-\widetilde{\Phi}(x-\delta)\big)+2\|f\|_\infty\,\widetilde{\Phi}(x-\delta) \\
& =\frac{1}{\alpha}-\psi(z)\,\widetilde{\Phi}(x-z)+\Big(2\|f\|_\infty+\psi(z)-\frac{1}{\alpha}\Big)\,\widetilde{\Phi}(x-\delta).
\end{split}
\end{equation*}
In view of the elementary inequality 
\begin{equation*}
\widetilde{\Phi}(x-\delta)\le\widetilde{\Phi}(x-z)\,\exp\bigg(\!-\frac{(\delta-z)(\delta+z-2x-2\Lambda_{t+n\Delta}+2\Lambda_t)}{2n\Delta}\bigg),
\end{equation*}
the latter cannot exceed 
\begin{equation}\label{case2bnd}
\frac{1}{\alpha}-\widetilde{\Phi}(x-z)\,\bigg(\psi(z)-\Big(2\|f\|_\infty+\psi(z)-\frac{1}{\alpha}\Big)_+\,\exp\bigg(\!-\frac{(\delta-z)(\delta+z-2x-2\Lambda_{t+n\Delta}+2\Lambda_t)}{2n\Delta}\bigg)\!\bigg).
\end{equation}

\smallskip

Combining $\mu\big((-\infty,x]\big)\ge\frac{1}{2}$, the second inequality in \eqref{ineq:comp} and the reflection principle for Brownian motion we find $\widetilde{\Phi}(x)\ge\frac{1}{4}$. In other words, $x\ge -\Lambda_{t+n\Delta}+\Lambda_t+\sqrt{n\Delta}\,q$, where $q$ is the $\frac{1}{4}$-quantile of the standard Gaussian distribution. Therefore, writing $\Phi$ for the standard Gaussian cumulative distribution function again, we conclude 
\begin{equation}\label{Gaussianbnd}
\widetilde{\Phi}(x-z)=\Phi\bigg(\frac{x-z+\Lambda_{t+n\Delta}-\Lambda_t}{\sqrt{n\Delta}}\bigg)
\ge\Phi\bigg(\frac{-z+\sqrt{n\Delta}\,q}{\sqrt{n\Delta}}\bigg)
=\Phi\bigg(\!-\frac{z}{\sqrt{n\Delta}}+q\bigg).
\end{equation}
In addition, recalling part (a), the minimality property \eqref{physical} and Lemma \ref{lemma:a priori} we obtain
\begin{equation*}
x\ge -\Lambda_{t+n\Delta}+\Lambda_t+q\,\sqrt{n\Delta}
\ge -\Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{n\Delta}\big)+q\,\sqrt{n\Delta}.
\end{equation*}
This yields 
\begin{equation*}
\Psi^{-1}\big(\Psi(-x)\big)-\Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{n\Delta}\big)\le -q\,\sqrt{n\Delta}
\end{equation*}
and, since $(\Psi^{-1})'\ge 1/\psi(\delta)$, 
\begin{equation}\label{SDbnd}
\Psi(-x)-\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{n\Delta}\le -q\,\sqrt{n\Delta}\,\psi(\delta)\quad\Longleftrightarrow\quad
\sqrt{n\Delta}\ge\frac{\Psi(-x)}{\|f\|_\infty\,\sqrt{2/\pi}-q\psi(\delta)}. 
\end{equation} 

\smallskip

Finally, we choose $z=0$ if $\psi(0):=\lim_{y\downarrow0} \psi(y)>0$ and $z=\frac{\delta}{2}$ if $\psi(0)=0$, and combine \eqref{case2bnd}, $\widetilde{\Phi}(x)\ge\frac{1}{4}$, \eqref{Gaussianbnd} and \eqref{SDbnd} to get the estimate
\begin{equation*}
\begin{cases}
\frac{1}{\alpha}-\frac{1}{4}\,\Big(\psi(0)-\big(2\|f\|_\infty+\psi(0)-\frac{1}{\alpha}\big)_+\,\exp\Big(\!-\frac{\delta(\delta-2x-2\Lambda_{t+n\Delta}+2\Lambda_t)}{2n\Delta}\Big)\Big) & \text{if}\;\;\;\psi(0)>0, \\
\frac{1}{\alpha}-\Phi\Big(q-\frac{\delta(\|f\|_\infty\,\sqrt{2/\pi}-q\psi(\delta))}{2\Psi(-x)}\Big) & \quad \\
\quad\;\;\;\,\cdot\Big(\psi(\delta/2)-\big(2\|f\|_\infty+\psi(\delta/2)-\frac{1}{\alpha}\big)_+\exp\Big(\!-\frac{\delta(3\delta/2-2x-2\Lambda_{t+n\Delta}+2\Lambda_t)}{4n\Delta}\Big)\Big) &
 \text{if}\;\;\;\psi(0)=0
\end{cases}
\end{equation*}
on the density of $\min_{0\le m\le n} X_{t+m\Delta}\,\mathbf{1}_{\{\tau>t\}}$ on $(-\delta,0)$ in the second case. (Note that the respective long parenthesis is non-negative thanks to $x\le 0$, $\Lambda_{t+n\Delta}-\Lambda_t\le\delta/6$, $n\Delta\le\teps$ and \eqref{teps:UBD}, as well as to $\psi(\delta/2)\le\frac{1}{\alpha}$ and $\Psi(\delta/6)\le\psi(\delta/2)\delta/6$ when $\psi(0)=0$.) We conclude the proof by using $x\le 0$, $\Lambda_{t+n\Delta}-\Lambda_t\le\delta/6$ and $n\Delta\le\teps$, and then putting the resulting bound together with the one found in the first case. (Hereby, $\frac{1}{4}\le\frac{1}{2}$ and $\psi\le\frac{1}{\alpha}$ are exploited.) \qed

\medskip

By combining Proposition \ref{prop:density_est}(a) with Lemma \ref{lemma:a priori} we can control the modulus of continuity of $\Lambda$ on right time neighborhoods. 

\begin{cor}\label{cor:mod_of_cont}
In the situation of Proposition \ref{prop:density_est}, it holds 
\begin{equation}
\Lambda_{s_2}-\Lambda_{s_1}\le 2\Psi^{-1}\big(\|f\|_\infty\,\sqrt{2/\pi}\,\sqrt{s_2-s_1}\big),\quad t\le s_1<s_2\le t+\frac{\pi}{8\|f\|_\infty^2}\,\Psi(\delta/6)^2.
\end{equation}
\end{cor}

\noindent\textbf{Proof.} It suffices to apply Lemma \ref{lemma:a priori} with $t=s_1$ upon recalling the density estimate of Proposition \ref{prop:density_est}(a) with $s=s_1$. \qed

%We first extend Theorem \ref{thm::kr} to show that convergence holds for a sufficiently small time interval provided the initial density falls in either category (\ref{cat_i}) or  (\ref{cat_ii}), without the more restrictive assumption \eqref{init_dens}.
%
%\begin{theorem}\label{thm_initial}
%	Assume that %$f$ is bounded on $[0,\infty)$ and
%	\begin{eqnarray}
%	\label{lim_x_0}
%	\lim_{x\downarrow0} f(x)<\frac{1}{\alpha}.
%	\end{eqnarray}
%	Then there exists $\teps>0$ such that %$\La^{\Delta} \rightarrow \La$ uniformly on $[0,\teps]$.
%	\[
%	\sup_{t \in [0,\teps]} |\La_t^{\Delta} - \La_t| \rightarrow 0.
%	\]
%\end{theorem}
%
%
%
%We first prove the following lemma.
%\begin{lemma}\label{lem1}
%	Under the assumptions of Theorem \ref{thm_initial},
%	there exist $\teps>0$, $x_0>0$, $1>\eta>0$, $M>0$, such that for all $0<x\le x_0$, increasing sequences $(t_j)_{0\le j\le n}$ with $t_0=0$ and $t_n=\teps$, and all $i$, $1\le i\le n$,
%	\begin{eqnarray}
%	\label{first_dens_inequ}
%	\mathbb{P}\left(-\alpha x < \min_{0\le j<i} X_{t_j} \le 0\right) &\le& \eta x, \\
%	\label{second_dens_inequ}
%	\mathbb{P}\left(0 < \min_{0\le j<i} X_{t_j} \le x\right) &\le& M x.
%	\end{eqnarray}
%\end{lemma}
%
%
%\begin{proof}
%	We start by proving the stricter first inequality \eqref{first_dens_inequ}.
%	As $0$ is a continuity point, $X_0 = X_{0-}$.
%	For $1<i<n$, let $\bar{V}_i = \min_{j < i} X_{t_j} - X_0 = \min_{j < i} \left(B_{t_j} - \La_{t_j} \right)$. Then
%	\begin{eqnarray*}
%		\mathbb{P}\left(-\alpha x < \min_{0\le j<i} X_{t_j} \le 0\right) &\le&
%		\int_{-\infty}^0 \mathbb{P}(X_0 \in (-\alpha x-v,-v)) \, \mathbb{P}(\bar{V}_i \in dv).
%	\end{eqnarray*}
%	
%	
%	By \eqref{lim_x_0}, there exist $1>\eta_0>0$, $v_0>0$ and $x_0>0$, such that
%	\begin{eqnarray}
%	\label{eq_v0_x0}
%	\mathbb{P}(X_0 \in (-\alpha x-v,-v)) \le \eta_0 x \qquad \forall 0<x<x_0, \,  -v_0<v<0.
%	\end{eqnarray}
%	Therefore,
%	\begin{eqnarray}
%	\label{first_int}
%	\int_{-v_0}^0 \mathbb{P}(X_0 \in (-\alpha x-v,-v)) \, \mathbb{P}(\bar{V}_i \in dv) \le \eta_0 x \qquad \forall 0<x<x_0.
%	\end{eqnarray}
%	Denoting the lowest upper bound on $f$ by $M$, we have
%	\begin{eqnarray}
%	\label{second_int}
%	\int_{-\infty}^{-v_0} \mathbb{P}(X_0 \in (-\alpha x-v,-v)) \, \mathbb{P}(\bar{V}_i \in dv) \le M \alpha x  \, \mathbb{P}(\bar{V}_i \le -v_0)
%	\qquad \forall 0<x,
%	\end{eqnarray}
%	and it remains to estimate the last term.
%	
%	As the map $t\rightarrow \La_t$ is increasing and $\min_{t \le t_i} B_{t} \le \min_{j < i} B_{t_j}$,
%	\begin{eqnarray*}
%		\mathbb{P}(\bar{V}_i \le -v_0) &=& \mathbb{P}(\min_{j < i} \left(B_{t_j} - \La_{t_j} \right) \le -v_0) \\
%		&\le&  \mathbb{P}(\min_{t\le t_i} B_{t} \le -v_0 +  \La_{t_i}).
%	\end{eqnarray*}
%	For $\teps$ small enough, by Theorem \ref{thm1} there exists $C>0$ such that 
%	\begin{eqnarray*}
%		0\le \La_t \le C \, t^{1/2}  \qquad \forall 0\le t \le \teps.
%	\end{eqnarray*}
%	Setting $v_0 = (K+1) C t_i^{1/2}$ for some $K>0$ to be determined, we have
%	\begin{eqnarray*}
%		\mathbb{P}(\bar{V}_i \le -v_0) &\le& \mathbb{P}(\min_{t\le t_i} B_{t} \le - K C t_i^{1/2}) \\
%		&=&  2 \mathbb{P}(B_{t_i} \le - K C t_i^{1/2}) \\
%		&=& 2  \Phi(- K C)
%	\end{eqnarray*}
%	by the reflection principle, with $\Phi$ the cumulative distribution function of the standard normal.
%	
%	Now we can first choose an $\eta_1$ such that $\eta_0 + \eta_1 <1$, then $K$ such that
%	$2  \Phi(- K C) \le \eta_1/(M \alpha)$, and finally $\teps$ such that $v_0 = (K+1) C t_i^{1/2}$
%	satisfies the requirements of \eqref{eq_v0_x0} for all $t_i\le \teps$.
%	Adding up \eqref{first_int} and \eqref{second_int} we obtain \eqref{first_dens_inequ}.
%	
%	For \eqref{second_dens_inequ}, we have directly
%	\begin{eqnarray*}
%		\mathbb{P}\left(0 < \min_{0\le j<i} X_{t_j} \le x \right) &\le&
%		\int_{-\infty}^0 \mathbb{P}(X_0 \in (-v,-v+x)) \, \mathbb{P}(\bar{V}_i \in dv) \\
%		&\le& M x.
%	\end{eqnarray*}
%	
%	
%	
%\end{proof}
%
%
%\begin{proof}
%	[Proof of Theorem \ref{thm_initial}]
%	
%	The proof is similar to the proof of Theorem 1 in \cite{KR}, but crucially replacing Lemma 3 in \cite{KR} by our generalised estimates from Lemma \ref{lem1}.
%	
%	To begin with, we note that the result from Lemma 1 in \cite{KR},
%	\begin{equation}
%	\label{asmussen_result}
%	\frac{1}{2 \sqrt{\Delta |\log(t/\Delta)|}} \sup_{s \le t} \left(X_{s}  - X^{*}_s \right)\rightarrow_{d}  1 \qquad \text{as } \Delta\to 0, %\sqrt{2 \log{\frac{t}{h}}} \qquad \text{as } h\to 0,
%	\end{equation}
%	for $X^{*}_t = X_0 + B_{\Delta \lfloor t/\Delta \rfloor} - \La_{\Delta \lfloor t/\Delta \rfloor}$,
%	still holds in our setting (one can retrace the steps in the proof there replacing the assumption \eqref{L_prime} on the derivative of $t\La$ by H\"older-1/2 continuity of $\La$).
%	
%	It is then also possible to deduce in a similar way to Lemma 2 in \cite{KR} that, for any $p < 1/2$, there exists $\gamma > 0$ independent of $\Delta$ and $i$ such that 
%	\begin{equation}
%	\label{eqn_1_2_delta}
%	0 \le \mathbb{P}\left(\min_{j < i} X_{t_j} > 0\right) -  \mathbb{P}\left(\inf_{s < t_i} X_s > 0\right)  \le  \gamma \Delta^p,
%	\end{equation}
%	by replacing in one step of the proof Lemma 2 in \cite{KR} the assertion of the existence of a bounded density for $\min_{j < i} X_{t_j} $ by \eqref{second_dens_inequ}.
%	
%	We now proceed by induction.
%	For $t_0 = 0$, we have $\La_0 = {\La}^\Delta_0$;  for $t_1$, we have
%	%$\min_{j < 1} \tilde{Y}_{t_j} = X_0$ and $\mathbb{P}(X_0 > 0) = 1$, hence 
%	from \eqref{eqn_1_2_delta},
%	\begin{equation*}
%	| {\La}^\Delta_{t_1} - \La_{t_1} | \le \left|  1 -  \mathbb{P}\left(\inf_{s < t_1} X_s > 0\right) \right| \le \gamma \Delta^p.
%	\end{equation*}
%	
%	For $i>1$, assume now that we have shown $\La^\Delta_{t_j} = \La_{t_j} - \tilde{C}_j \Delta^p$ for $j < i$,
%	where ${C}_j \ge 0$ as ${\La}^\Delta_{t_j} \le \La_{t_j}$. 
%	We split the error into two contributions, % to be analysed separately,
%	\begin{eqnarray}
%	\nonumber
%	&&|{\La}^\Delta_{t_i} - \La_{t_i} | = \left| \mathbb{P}\left(\min_{j < i} {X}^\Delta_{t_j} > 0\right) - \mathbb{P}\left(\inf_{s < t_i} X_s > 0\right) \right| \\
%	&&\hspace{-1 cm} \le \left| \mathbb{P}\left(\min_{j < i} {X}^{\Delta}_{t_j}> 0\right) - \mathbb{P}\left(\min_{j < i}  X_{t_j} > 0\right)  \right| + \left|  \mathbb{P}\left(\min_{j < i} X_{t_j} > 0\right) -  \mathbb{P}\left(\inf_{s < t_i} X_s > 0\right) \right|.
%	\label{two-parts}
%	\end{eqnarray}
%	%We can use Lemma \ref{lemma_1_2_delta}, (\ref{eqn_1_2_delta}), for the second term.
%	For the first term,
%	\begin{eqnarray*}
%		\mathbb{P}\left(\min_{j < i} {X}^\Delta_{t_j}> 0\right) -  \mathbb{P}\left(\min_{j < i}X_{t_j} > 0\right) && \\
%		&\hspace{-4 cm}=& \hspace{-2 cm} \mathbb{P}\left(\min_{j < i} \left(X_{t_j} + {C}_j \Delta^p   \right) > 0\right) - \mathbb{P}\left(\min_{j < i} X_{t_j} > 0\right)    \\
%		&\hspace{-4 cm}\le& \hspace{-2 cm} \mathbb{P}\left(\min_{j < i} X_{t_j}   >  - \max_{j < i} {{C}_j} \Delta^p \right) - \mathbb{P}\left(\min_{j < i} X_{t_j} > 0\right) \\
%		&\hspace{-4 cm}\le& \hspace{-2 cm}   \eta \max_{j < i} {{C}_j} \Delta^p,
%	\end{eqnarray*}
%	by \eqref{first_dens_inequ}, with $\eta<1$.
%	Using \eqref{eqn_1_2_delta} to bound the second term in \eqref{two-parts}, we have %the following inequality for ${C}_i$,
%	\begin{equation*}
%	{C}_i \le \eta \max_{j < i} {C}_j + \gamma,
%	\end{equation*}
%	hence ${C}_i$ is bounded independent of $i$ and $\Delta$.
%	By induction we get the uniform convergence.
%\end{proof}
%
%\begin{remark}
%	From the proof of Theorem \ref{thm_initial} it follows that convergence of order $p$ still holds in this setting for all $p<1/2$.
%\end{remark}
%
%%It was shown in Propositions 2.1 and 4.1 of \cite{DNS} that the property (\ref{init_dens}) 
%%holds for 
%%{\color{blue}
%%	\sout{all times $t$ for which $L$ is continuous}
%%	all class (i) points above}, given some conditions on $Y_0$, 
%%in the following sense: {\color{blue} \fbox{Following theorem not stated correctly -- need to change.} }
%%\begin{theorem}[Delarue, Nadtochiy, Shkolnikov]\label{thm::dns_density}
%%	Under the same hypothesis as Theorem \ref{thm::dns_uniq}, the assumption in Theorem \ref{thm::kr} holds with $\beta = 1$ for the law of $Y_t \BONE_{\inf_{s < t} Y_s > 0}$, for all times $t$ where $Y$ and $L$ are continuous.
%%	That is, for every time $t$ where $\lim_{s \to t^-} L_s = L_t$, there is some $B$ for which 
%%	\[
%%	\BPP \left( Y_t \BONE_{\inf_{s < t} Y_s > 0} \in (0, x) \right) < Bx
%%	\]
%%	for sufficiently small $x > 0$.
%%\end{theorem}
%%

%%%%%%%%%%%%%%%%%
\subsection{Useful definitions}\label{subsec:M1}
%%%%%%%%%%%%%%%%% 

In this subsection, we prepare the definitions of the Skorokhod M1 convergence for non-decreasing functions and of some auxiliary time-stepping schemes used in the proof of Theorem \ref{thm::main}. 

%The main goal of this article is to % prove Theorem \ref{thm::main}. This extends 
%extend Theorem \ref{thm_initial} to all times $t$, and without the assumption \eqref{lim_x_0}.
%, i.e.\ show convergence for any initial density satisfying the mild Assumption \ref{ass}. 
%Kaushansky and Reisinger proved a partial extension of their theorem in the following sense: \cite{KR}
%\begin{theorem}\label{thm::kr_extend}
%Assume that we may choose $T$ in Theorem \ref{thm::kr} such that 
%\[
%2\alpha \left( \hat{B}T^{-\frac{1-\beta}{2}} + \frac{1}{\sqrt{T}} \right) < 1.
%\]
%Then, the bounds in Theorem \ref{thm::kr} hold up to any time $T' < j$, where $j$ the first time when $L$ is discontinuous.
%\end{theorem}
%
%We attempt to extend this result to a sense of convergence for all times. 
%However, %the statement of Theorem \ref{thm::kr} 
%uniform convergence
%cannot possibly hold for all times past a point of discontinuity, because the size of the discontinuity does not depend on the time step. We thus define -- and subsequently prove convergence in -- the Skorokhod M1 topology.

\begin{dfn}[see, e.g., \cite{Whi}, Corollary 12.5.1]\label{M1def}
Let $T>0$. A sequence $(L_k)_{k\in\mathbb{N}}$ of non-decreasing functions in $D([0,T])$ is said to \emph{converge in M1 sense} to some $L\in D([0,T])$ if and only if $\lim_{k\to\infty} L_k(t)=L(t)$ for all $t$ in a dense subset of $[0,T]$ that includes $0$ and $T$. 
\end{dfn}

%\begin{definition}[Skorokhod M1 Topology]\label{defn::m1}
%	Given a cadlag function $f: [0, \infty) \to \BRR$, let its points of discontinuity be $t_1, t_2, \dots$. Define the curve of $f$ to be the continuous path that connects the discontinuities, in the following sense: for every integer $i$, define $\gamma: [0, \infty) \to \BRR^2$ such that
%	\[
%	\gamma(2i + m) = (t_i + m(t_{i+1} - t_i), f(t_i + m(t_{i+1} - t_i))) \quad \textnormal{for} \quad m \in [0, 1),
%	\]
%	and
%	\[
%	\gamma(2i + 1 + m) = (t_{i+1}, f(t_{i+1}^-) + m(f^-(t_{i+1}) - f^-(t_{i+1}))) \quad \textnormal{for} \quad m \in [0, 1),
%	\]
%	where $f(t_{i+1}) = \lim_{s \to t_{i+1}^-} f(s)$. 
%Intuitively, this is the path drawn out by connecting the discontinuities together.
	
%	Then, define the distance between two such functions $f, g$, with associated curves $\gamma_f, \gamma_g$, to be 
%	\[
	%d(f, g) := \inf_{\phi \in C(\BRR), \textnormal{ increasing}} \sup_{x \ge 0} d_{\BRR^2}(\gamma_f(\phi(x)), \gamma_g(x)),
%	d(f, g) := \inf \left\{\sup_{x \ge 0} d_{\BRR^2}(\gamma_f(\phi(x)), \gamma_g(x)), \; \phi \in C(\BRR) \textnormal{ increasing}\right\},
%	\]
%	where $d_{\BRR^2}: \BRR^2 \times \BRR^2 \to \BRR$ is the usual distance function on $\BRR^2$.
	
%\end{definition}



%\section{Outline of Proof of Theorem \ref{thm::main}}

%In the main part of the proof, we show that under the hypotheses of Theorem \ref{thm::main}, for every $\epsilon$, there exists some $\Delta$ such that $d(L, L^\Delta) < \epsilon$, up to the first accumulation point. From this we will deduce that this holds for all sufficiently small $\epsilon$.
%% NEED TO EDIT THIS AS APPROPRIATE
%

\begin{dfn}\label{defn::discrete_general}
\begin{enumerate}[(a)]	
\item Given $t\ge0$, $\Delta>0$, a physical solution $\Lambda$ and the associated $X$, we define $X^{t;\Delta}_{t+n\Delta}$, $n=0,\,1,\,\ldots$ and $\Lambda^{t;\Delta}_{t+n\Delta}$, $n=1,\,2,\,\ldots$ recursively by $X^{t;\Delta}_t=X_t$, 
\begin{equation}
\begin{split}
& \Lambda^{t;\Delta}_{t+n\Delta}=\alpha\pp\Big(\inf_{0\le s\le t} X_s\le 0\;\,\text{or}\,
\min_{0\le m\le n-1} X^{t;\Delta}_{t+m\Delta}<0\Big),\;n=1,2,\ldots\;\;\text{and} \\ 
& X^{t;\Delta}_{t+n\Delta}=X_{0-}+B_{t+n\Delta}-\Lambda^{t;\Delta}_{t+n\Delta},\;n=1,2,\ldots.  
\end{split}
\end{equation}
We extrapolate by setting $\Lambda^{t;\Delta}_{0-}=0$, $\Lambda^{t;\Delta}_s=\Lambda_s$, $s\in[0,t]$ and $\Lambda^{t;\Delta}_s=\Lambda^{t;\Delta}_{\max\{t+n\Delta:\,t+n\Delta\le s\}}$, $s>t$, as well as $X^{t;\Delta}_{0-}=X_{0-}$ and $X^{t;\Delta}_s = X_{0-} + B_s - \Lambda^{t;\Delta}_s$, $s\ge 0$. 
\item Given a sequence $\CTT$ of the form $0=t_0<t_1<t_2<\cdots$, we let $X^{\CTT}_{t_n}$, $n=0,\,1,\,\ldots$ and $\Lambda^{\CTT}_{t_n}$, $n=1,\,2,\,\ldots$ be defined recursively by $X^{\CTT}_{t_0}=X_0$, 
\begin{equation}
\Lambda^{\CTT}_{t_n}=\alpha\pp\Big(\min_{0\le m\le n-1} X^{\CTT}_{t_m}<0\Big),\;n=1,2,\ldots\;\;\text{and}\;\;\, X^{\CTT}_{t_n}=X_{0-}+B_{t_n}-\Lambda^{\CTT}_{t_n},\;n=1,2,\ldots.  
\end{equation}
We extrapolate by setting $\Lambda^{\CTT}_{0-}=0$, $\Lambda^{\CTT}_0=\alpha\pp(X_0\le0)$ and $\Lambda^{\CTT}_t=\Lambda^{\CTT}_{\max\{t_n:\,t_n\le t\}}$, $t>0$, as well as $X^{\CTT}_{0-}=X_{0-}$ and $X^{\CTT}_t = X_{0-} + B_t - \Lambda^{\CTT}_t$, $t\ge0$. 
\end{enumerate}
\end{dfn}

\begin{rmk}\label{rmk::discrete_general_prelim}
If $\CTT,\widetilde{\CTT}$ are sequences as in Definition \ref{defn::discrete_general}(b) and $\CTT$ is a subsequence of $\widetilde{\CTT}$, then $\La^{\CTT}\le\La^{\widetilde{\CTT}}\le\La$, by induction. 
\end{rmk}

%\textcolor{red}{We first show that we can extend convergence forward in time past any continuity point $t$.
%, then we also have convergence on $[0,t+\delta]$ for small enough $\delta>0$.
%a form of Theorem \ref{thm::kr} without the imposed conditions (\ref{init_dens}), (\ref{L_prime}) and (\ref{cond_T}), and up to the first
%discontinuity.
%This is essentially achieved through %repeated 
%application of Theorem \ref{thm_initial}, proving a new stability property of the scheme and using the regularity at the ``re-start'' ascertained by Theorem \ref{thm1}. 
%This is completed in Section \ref{sec::no_jump}. Next, we establish a similar extension property past any point $t$ where $\La$ is discontinuous.
%The main difficulty arises from the fact that the discrete boundary approximation ``jumps'' after the true boundary. 
%This extension is achieved in Section \ref{sec::special_case} by showing that we can find a time $k_\Delta > t$ (depending on $\Delta$) such that we 
%have
%\[
%d(L|_{[0, k_\Delta]}, L^{\Delta}|_{[0, k_\Delta]}) \to 0,
%\]
%in the sense that for every $\epsilon > 0$, for sufficiently small $\Delta$, we 
%may find $k_\Delta > t$ such that
%\[
%d(\La|_{[0, k_\Delta]}, \La^{\Delta}|_{[0, k_\Delta]}) < \epsilon.
%\]
%Next, in Section \ref{sec::post_jump}, we use induction on the number of points of discontinuity to conclude the proof of Theorem 5.
%In Section \ref{sec::post_jump} we complete the proof using these two main steps.}

==> arXiv v2/Section4_final_v2.tex <==
%!TEX root =Main.tex
\newcommand{\ep}{\hfill \ensuremath{\Box}}

\section{Proof of Theorem \ref{thm::main}} \label{sec:mainproof}

For the proof of the convergence globally in time (Theorem \ref{thm::main}), we prepare auxiliary error propagation bounds in Subsection \ref{sec::stab} and then show respectively that the convergence can be extended beyond continuity and discontinuity points of $\Lambda$ in Subsections \ref{sec::no_jump} and \ref{sec::special_case}.
%For the purposes of our analysis, it will be useful to consider a broader class of discrete processes, which includes $\La^\Delta$ from Definition \ref{defn::discrete}. 
%\begin{definition}\label{defn::discrete_general}
%	Let $\CTT = (t_1, t_2, \dots)$ be an increasing sequence of positive numbers. We define the processes $\La^{\CTT}, X^{\CTT}$ in the following manner:
%	\begin{equation}\label{eq::discrete_general}
%		X^{\CTT}_{t_i} = X_0 + B_{t_i} - \La^{\CTT}_{t_i}, \qquad \La^{\CTT}_{t_i} = \alpha \BPP \left( \inf_{j < i} X^{\CTT}_{t_j} < 0 \right).
%	\end{equation}
%	As in Definition \ref{defn::discrete}, we extrapolate $\La^{\CTT}_s = \La^{\CTT}_{t_i}$ and $X^{\CTT}_s = X_0 + B_s - \La^{\CTT}_s$ for $s \in [t_i, t_{i+1})$.
%\end{definition}
%
%\begin{remark}\label{rmk::discrete_general_prelim}
%	We have that $\La^\Delta = \La^{\CTT}$ for $\CTT = (\Delta, 2\Delta, \dots)$. For sequences $\CTT$ and $\CTT'$ such that $\CTT$ is a subsequence of $\CTT'$, we have $\La^{\CTT'} \ge \La^{\CTT}$, by induction. Because we also have $\La \ge \La^\Delta$, this implies $d_{\mathrm{M1}}(\La, \La^{\CTT}) \ge d_{\mathrm{M1}}(\La, \La^\Delta)$ for every $\Delta, \CTT$ such that $t_i/\Delta \in \mathbb{Z}$ for all $i$.
%\end{remark}
\subsection{Auxiliary error propagation bounds} \label{sec::stab}
%For our proof of Proposition \ref{pro::no_jump} we need 
The following lemma gives an estimate concerning the continuity of the numerical solution with respect to the initial condition.
%difference between the increments of two approximating functions $\Lambda^\Delta$ and $\widetilde{\Lambda}^\Delta$, as introduced in Definition \ref{defn::discrete}, in terms of the difference between the associated initial values $X^\Delta_0$ and $\widetilde{X}^\Delta_0$.  
The statement is weaker than typical notions of stability as the ``constant'' in it may depend on $\Delta$, but this is sufficient for our purposes.

\begin{lem}\label{lem::discrete_compare}
For some $\Delta>0$ and $K\ge0$, let $(X^\Delta, \Lambda^\Delta)$ be given by Definition \ref{defn::discrete}, and let $\widetilde{X}^\Delta_{n\Delta}$, $n=0,\,1,\,\ldots$ and $\widetilde{\Lambda}^\Delta_{n\Delta}$, $n=0,\,1,\,\ldots$ be defined by $\widetilde{X}^\Delta_0=X^\Delta_0+K$, $\widetilde{\Lambda}^\Delta_0=\alpha\mathbb{P}(\widetilde{X}^\Delta_0\le0)$, 
\begin{equation}
\widetilde{\Lambda}^{\Delta}_{n\Delta}=\alpha\pp\Big(\min_{0\le m\le n-1} \widetilde{X}^\Delta_{m\Delta}<0\Big),\;n\ge 1\;\;\text{and}\;\; \widetilde{X}^\Delta_{n\Delta}=\widetilde{X}^\Delta_0+B_{n\Delta}-\widetilde{\Lambda}^\Delta_{n\Delta}
+\widetilde{\Lambda}^\Delta_0
,\;n\ge 1.  
\end{equation}
We extrapolate to $t>0$ by setting $\widetilde{\Lambda}^{\Delta}_t=\widetilde{\Lambda}^{\Delta}_{\lfloor t/\Delta \rfloor \Delta}$ and $\widetilde{X}^{\Delta}_t=\widetilde{X}^{\Delta}_{\lfloor t/\Delta \rfloor \Delta}$. If $X_{0-}\ge0$ admits a density on $[0,\infty)$, then for any $T>0$, there is some $C=C_\alpha(\Delta,T)\ge0$ non-decreasing in $\alpha$ and non-increasing in $\Delta$ such that
\begin{equation}
(\Lambda^\Delta_t-\Lambda^\Delta_0)-(\widetilde{\Lambda}^\Delta_t-\widetilde{\Lambda}^\Delta_0)\leq CK,\quad t\in[0,T].
\end{equation}
\end{lem}

\noindent\textbf{Proof.} For $n\!\ge\!1$, by $\min_{0\le m \le n-1} \widetilde{X}^\Delta_{m\Delta}\!\ge0\Leftrightarrow\widetilde{X}^\Delta_{m\Delta}\ge0,\,0\!\le\! m\!\le\! n\!-\!1$ and the union bound
\begin{equation*}
\begin{split}
\BPP \Big( \min_{0\le m \le n-1} X^\Delta_{m\Delta} < 0 \le \min_{0\le m \le n-1} \widetilde{X}^\Delta_{m\Delta} \Big) &\le\,
\BPP \Big(\exists\,0\le m\le n-1:\; X^\Delta_{m\Delta} < 0 \le \widetilde{X}^\Delta_{m\Delta}\Big) \\
&\le\,\sum_{m=0}^{n-1} \BPP \big( X^\Delta_{m\Delta} < 0 \le \widetilde{X}^\Delta_{m\Delta} \big).
\end{split}
\end{equation*}
Now, we set $K_n=(\Lambda^\Delta_{n\Delta}-\Lambda^\Delta_0)-(\widetilde{\Lambda}^\Delta_{n\Delta}-\widetilde{\Lambda}^\Delta_0)$, $n=1,\,2,\,\ldots\,$. Then, using the latter estimate and bounding the standard normal density by its maximum we infer
\begin{equation*}
\begin{split}
& \; K_n \le \alpha\pp\Big( \min_{0\le m \le n-1} X^\Delta_{m\Delta} < 0 \le \min_{0\le m \le n-1} \widetilde{X}^\Delta_{m\Delta} \Big)-\alpha\pp\big(X^\Delta_0\le 0<\widetilde{X}^\Delta_0\big) \\
& \le \sum_{m=1}^{n-1} \alpha\pp\big(X^\Delta_{m\Delta} < 0 \le \widetilde{X}^\Delta_{m\Delta} \big) 
=\sum_{m=1}^{n-1} \alpha\pp\Big( B_{m\Delta} \in \big[\widetilde{\Lambda}^\Delta_{m\Delta} -\widetilde{\Lambda}^\Delta_0-\widetilde{X}^\Delta_0,\Lambda^\Delta_{m\Delta} -\Lambda^\Delta_0-X^\Delta_0\big)\Big) \\
& \le \sum_{m=1}^{n-1} \frac{\alpha}{\sqrt{2\pi m\Delta}} (K_m + K).
\end{split}
\end{equation*}
By induction, we conclude that $K_n\le \widehat{C}_\alpha(\Delta,n)K$, $n=1,\,2,\, \ldots\,$, for suitable constants $\widehat{C}_\alpha(\Delta,n)\ge0$, $n=1,\,2,\,\ldots\,$.
It remains to take $C_\alpha(\Delta,T)=\max_{1\le n \le \lceil T/\Delta\rceil} \widehat{C}_\alpha(\Delta,n)$. \ep
	
\medskip

%As a consequence of Lemma \ref{lem::discrete_compare}, we can compare the increments beyond a time $s\ge0$ of functions extended from $[0,s]$ to $[0,\infty)$ via an analogue of Definition \ref{defn::discrete}. In particular, we consider a discrete extension of the free boundary $\Lambda_q$, $q\in[0,s]$ to $[0,\infty)$, defined next.
%
%\begin{definition}\label{defn::continuous_then_discrete}
%For $s\ge0$ and a  physical solution $(X,\Lambda)$ of \eqref{eq::init1}--\eqref{eq::init2}, we define the pair $(X^{s,\Delta},\Lambda^{s,\Delta})$ by 
%\begin{eqnarray}
%(X^{s,\Delta}_q,\Lambda^{s,\Delta}_q) &=& (X_q,\Lambda_q), \quad q\in[0,s], \\ 
%\Lambda^{s, \Delta}_{s+n\Delta} &=& \alpha\pp\Big(\min\Big(\min_{q\in[0,s]} X_q,\min_{0\le m\le n-1} X^{s,\Delta}_{s+m\Delta}\Big) \le 0\Big), \quad n=1,\,2,\,\ldots, \\
%X^{s, \Delta}_{s + n\Delta} &=& X_{0-} + B_{s + n\Delta} - \Lambda^{s, \Delta}_{s + n\Delta},\quad n=1,\,2,\,\ldots,
%\end{eqnarray}
%and the extrapolations $\Lambda^{s, \Delta}_{s + r} = \Lambda^{s, \Delta}_{s+\lfloor r /\Delta\rfloor\Delta}$, $r\ge0$ and $X^{s, \Delta}_{s+r} = X_{0-} + B_{s+r} - \Lambda^{s, \Delta}_{s+r}$, $r\ge0$.  
%\end{definition}

The extension proofs in Subsections \ref{sec::no_jump}, \ref{sec::special_case} rely on the following corollary of Lemma \ref{lem::discrete_compare}.
%of Proposition \ref{pro::no_jump} and is used again in Section \ref{sec::special_case} below (for the extension beyond a discontinuity point). 

\begin{cor}\label{cor::discrete_compare}
For every $\Delta>0$ and $0\le r\le s$, there is some $C=C_\alpha(\Delta,s-r)\ge0$ non-increasing in $\Delta$ such that for any $N\ge0$ and sequence $\CTT$ of the form 
\begin{equation*}
0=t_0<\cdots<t_N=r<r+\Delta<r+2\Delta<\cdots, 
\end{equation*}
the function $\Lambda^{r;\Delta}$ from Definition \ref{defn::discrete_general}(a) and the function $\Lambda^{\CTT}$ from Definition %\ref{defn::continuous_then_discrete} 
\ref{defn::discrete_general}(b) satisfy
\begin{equation}
\Lambda^{r;\Delta}_{r+t}-\Lambda^{\CTT}_{r+t}\le C (\Lambda^{r;\Delta}_r-\Lambda^{\CTT}_r) ,\quad t\in[0,s-r],
\end{equation}
provided $X_{0-}\ge0$ admits a density on $[0,\infty)$. 
%where $K:=\Lambda^{s,\Delta}_s-\Lambda^{\CTT}_s$.    
\end{cor}

\noindent\textbf{Proof.} We first note the comparison of increments
\begin{equation}\label{incr_comp}
\Lambda^{\CTT}_{r+t} - \Lambda^{\CTT}_r \ge \widetilde{\Lambda}^{r;\Delta}_{r+t} - \widetilde{\Lambda}^{r;\Delta}_r,\quad t\in[0,s-r], 
\end{equation} 
where $(\widetilde{X}^{r;\Delta}_{r+t},\widetilde{\Lambda}^{r;\Delta}_{r+t})$, $t\in[0,s-r]$ is defined by $\widetilde{X}^{r;\Delta}_r=X^{\CTT}_r$, $\widetilde{\Lambda}^{r;\Delta}_r=\alpha\pp\big(\inf_{0\le q\le r} X_q\le 0\big)$,
\begin{eqnarray*}
&& \widetilde{\Lambda}^{r;\Delta}_{r+n\Delta} = \alpha\pp\Big(\inf_{0\le q\le r} X_q\le 0\;\,\mathrm{or}\;
\min_{0\le m\le n-1} \widetilde{X}^{r;\Delta}_{r+m\Delta}<0\Big), \quad n=1,\,2,\,\ldots,\big\lfloor(s-r)/\Delta\big\rfloor,  \\
&& \widetilde{X}^{r;\Delta}_{r+n\Delta} = \widetilde{X}^{r;\Delta}_r + B_{r+n\Delta} - B_r - \widetilde{\Lambda}^{r;\Delta}_{r+n\Delta}+\widetilde{\Lambda}^{r;\Delta}_r,\quad n=1,\,2,\,\ldots,\,\big\lfloor(s-r)/\Delta\big\rfloor,
\end{eqnarray*}
and the extrapolations $\widetilde{\Lambda}^{r;\Delta}_{r+t} = \widetilde{\Lambda}^{r;\Delta}_{r+\lfloor t /\Delta\rfloor\Delta}$ and $\widetilde{X}^{r;\Delta}_{r+t} = \widetilde{X}^{r;\Delta}_{r+\lfloor t /\Delta\rfloor\Delta}$ for $t\in(0,s-r]$. Indeed, \eqref{incr_comp} is trivial for $t\in[0,\Delta)$ and holds for $t\in[\Delta,s-r]$, since 
\begin{equation}
\pp\Big(\min_{0\le m\le (N-1)_+} X^{\CTT}_{t_m}\!\ge 0,\,\min_{0\le m\le n-1} X^{\CTT}_{r+m\Delta}\!<0\Big) 
\ge \pp\Big(\inf_{0\le q\le r} X_q\!>0,\,\min_{0\le m\le n-1} \widetilde{X}^{r;\Delta}_{r+m\Delta}\!<0\Big),  
\end{equation}
$n:=\lfloor t /\Delta\rfloor=1,\,2,\,\ldots,\,\lfloor(s-r)/\Delta\rfloor$, as can be readily seen by induction.

\medskip

Conditioning on the event $\{\inf_{0\le q\le r} X_q>0\}$, which has probability $1-\Lambda_r/\alpha$, we get
\begin{eqnarray*}
&& \Lambda^{r;\Delta}_{r+t}-\Lambda^{r;\Delta}_r=(\alpha-\Lambda_r)\,\pp\Big(\min_{0\le m\le \lfloor t /\Delta\rfloor-1} X^{r;\Delta}_{r+m\Delta}\le 0\,\Big|\,\inf_{0\le q\le r} X_q>0\Big),\quad t\in[0,s-r], \\
&& \widetilde{\Lambda}^{r;\Delta}_{r+t}-\widetilde{\Lambda}^{r;\Delta}_r=(\alpha-\Lambda_r)\,\pp\Big(\min_{0\le m\le \lfloor t /\Delta\rfloor-1} \widetilde{X}^{r;\Delta}_{r+m\Delta}\le 0\,\Big|\,\inf_{0\le q\le r} X_q>0\Big),\quad t\in[0,s-r]. 
\end{eqnarray*} 
Thus, under the conditional measure $\pp(\,\cdot\,|\,\inf_{0\le q\le r} X_q>0)$, the pairs $(X^{r;\Delta}_{r+\cdot},\Lambda^{r;\Delta}_{r+\cdot}-\Lambda^{r;\Delta}_r)$ and $(\widetilde{X}^{r;\Delta}_{r+\cdot},\widetilde{\Lambda}^{r;\Delta}_{r+\cdot}-\widetilde{\Lambda}^{r;\Delta}_r)$ fit into the framework of Lemma \ref{lem::discrete_compare}, which yields the estimate
\begin{equation} \label{bound_from_lemma}
(\Lambda^{r;\Delta}_{r+t}-\Lambda^{r;\Delta}_r)-(\widetilde{\Lambda}^{r;\Delta}_{r+t}-\widetilde{\Lambda}^{r;\Delta}_r)\le C_{\alpha-\Lambda_r}(\Delta,s-r) K\le C_\alpha(\Delta,s-r) K,\quad t\in[0,s-r],\;\;\;
\end{equation}
where $K:=\Lambda^{r;\Delta}_r-\Lambda^{\CTT}_r=X^{\CTT}_r-X^{r;\Delta}_r=\widetilde{X}^{r;\Delta}_r-X^{r;\Delta}_r$. Using this definition of $K$, then \eqref{incr_comp}, and finally \eqref{bound_from_lemma}, we end up with
\begin{equation*}
\begin{split}
\Lambda^{r;\Delta}_{r+t}-\Lambda^{\CTT}_{r+t}
&=(\Lambda^{r;\Delta}_{r+t}-\Lambda^{r;\Delta}_r)-(\Lambda^{\CTT}_{r+t}-\Lambda^{\CTT}_r)+K \\
&\le (\Lambda^{r;\Delta}_{r+t}-\Lambda^{r;\Delta}_r)-(\widetilde{\Lambda}^{r;\Delta}_{r+t} - \widetilde{\Lambda}^{r;\Delta}_r)+K 
\le\big(C_\alpha(\Delta,s-r)+1\big)K. \qquad\qquad\quad\;\;\;\ep
\end{split}
\end{equation*}
	
%\chrb{Check if number of epsilons can be removed.}

\subsection{Extension beyond continuity points} \label{sec::no_jump}

We proceed to the following extension result.
%$\mathbb{T}$ defined at the end of the previous section, and $\mathbb{T}^{\rm (i)}$ and $\mathbb{T}^{\rm (ii)}$ defined in Theorem \ref{thm1}.


%that whenever $\Lambda^\Delta\underset{\Delta\downarrow0}{\longrightarrow}\Lambda$ in the M1 sense on an interval $[0,T)$, where $T\ge0$ is a continuity point of $\Lambda$, we must also have  $\Lambda^\Delta|_{[0,T+\delta]}\underset{\Delta\downarrow0}{\longrightarrow}\Lambda|_{[0,T+\delta]}$ in the M1 sense, for some $\delta>0$. The next proposition formalizes this statement.  %a variant of Theorem \ref{thm::kr_extend}.
%

%\begin{definition}\label{defTT}
%\end{definition}

\begin{prop}\label{pro::no_jump}
%Let $T \in \mathbb{T} \cap (\mathbb{T}^{\rm (i)} \cup \mathbb{T}^{\rm (ii)})$. 
Suppose Assumption \ref{ass}. Let $T\ge0$ be a continuity point of $\Lambda$ such that $\Lambda^\Delta|_{[0,t]}\underset{\Delta\downarrow0}{\overset{\emph{M1}}{\longrightarrow}}\Lambda|_{[0,t]}$ for any continuity point $t\in(0,T)$ of $\Lambda$. Then,  $\Lambda^\Delta|_{[0,T+\teps]}\underset{\Delta\downarrow0}{\overset{\emph{M1}}{\longrightarrow}}\Lambda|_{[0,T+\teps]}$ for all $\teps>0$ small enough.
\end{prop}

\noindent\textbf{Proof.} We first argue that $\Lambda^\Delta|_{[0,T]}\underset{\Delta\downarrow0}{\overset{\text{M1}}{\longrightarrow}}\Lambda|_{[0,T]}$ if $T>0$. Thanks to the definition of the M1 convergence for monotone functions (Definition \ref{M1def}) and in view of the assumed convergence $\Lambda^\Delta|_{[0,t]}\underset{\Delta\downarrow0}{\overset{\text{M1}}{\longrightarrow}}\Lambda|_{[0,t]}$ for all continuity points $t\in(0,T)$ of $\Lambda$, it suffices to verify that $\lim_{\Delta\downarrow0} \Lambda^\Delta_T = \Lambda_T$. Taking a sequence $T_N\uparrow T$ as $N\to\infty$ satisfying $\lim_{\Delta\downarrow0}  \Lambda^\Delta_{T_N} = \Lambda_{T_N}$, $N=1,\,2,\,\ldots$ we obtain
\begin{equation}
\Lambda_T \ge \limsup_{\Delta\downarrow0}  \Lambda^\Delta_T 
\ge \liminf_{\Delta\downarrow0}  \Lambda^\Delta_T
\ge \lim_{\Delta\downarrow0}  \Lambda^\Delta_{T_N}=\Lambda_{T_N},\quad N=1,\,2,\,\ldots.
\end{equation}   
Since $\Lambda_{T_N}\uparrow \Lambda_T$ as $N\to\infty$, it must hold
\begin{equation}
\label{conv_T}
\Lambda_T=\lim_{\Delta\downarrow0}  \Lambda^\Delta_T.
\end{equation}  

\smallskip
%\medskip
%We 
%%{\color{blue} first consider the case $s<\inf \BTT^{({\rm ii})}$ and}
%argue by contradiction. Define the set of times $\BTT$ to contain all times $s$ in $[0, j)$ such that for every $\epsilon$, there exists some $\Delta_*$ (depending on $s$ and $\epsilon$) such that for all $\Delta < \Delta_*$, we have that
%	\[
%	L_u - L^\Delta_u < \epsilon,
%	\]
%	for all $u \in [0, s]$. Let $s' = \inf (([0, j) \backslash \BTT))$. By Theorems \ref{thm::kr} and \ref{thm::dns_density}, we have that $s' > 0$. If $s' = j$, then we are done; thus, assume for sake of contradiction that $s' < j$.
%	We first show that $s' \in \BTT$, and then that a right neighborhood of $s'$ is also in $\BTT$, giving us the desired contradiction.
%	
%	%{\color{blue} \cap \BTT^{({\rm i})}}
%	
%	
%	\textbf{Step 1: $s' \in \BTT$.}
%	Choose any $\epsilon > 0$. Since $L$ is continuous in a neighborhood of $s'$, we may find $s < s'$ such that $L_{s'} - L_s < \epsilon / 2$, and by definition of $\BTT$, we may find some $\Delta_*$ such that 
%	\[
%	L_u - L^\Delta_u < \epsilon/2.
%	\]
%	for $\Delta < \Delta_*$ and $u \in [0, s]$. This choice of $\Delta_*$ suffices, because for any $u \in [s, s']$, we have that 
%	\[
%	L_u - L^\Delta_u \le L_{s'} - L^\Delta_s < \epsilon,
%	\]
%	as desired.
%\noindent\textbf{There is some $\delta$ such that $[s', s' + \delta) \in \BTT$.}
%	We first consider the case that $T \in \BTT^{({\rm i})}$, and return to the case $T \in \BTT^{({\rm ii})}$ at the end.	
%In order to prove Step 2 of Proposition \ref{pro::no_jump}, 
%We apply Corollary \ref{cor::discrete_compare} to our current situation. 
%We assumed that $s'$ is a point in $\BTT$, and we seek to show that $[s', s' + \delta) \in \BTT$ for some $\delta$.
Next, we use Propositions \ref{thm1} and \ref{prop:density_est}(a) to find an $\teps>0$ such that \eqref{loc_rate_conv} applies to all $T\le t\le T+\teps$ with this $\teps$. To conclude we argue that $\lim_{\Delta\downarrow0} \Lambda^\Delta_s=\Lambda_s$, $s\in(T,T+\teps]$. Indeed, for every $\eta>0$, there exists a $\overline{\Delta}_0>0$ with the property 
\begin{equation}\label{Delta1}
\sup_{s\in[t,t+\teps]} |\Lambda^{t;\Delta_0}_s-\Lambda_s|\le\frac{\eta}{2},\quad T\le t\le T+\teps,\quad \Delta_0\in(0,\overline{\Delta}_0]. 
\end{equation}
%By Propositions \ref{thm1} and \ref{prop:density_est} (see also \cite[Theorem 1.1]{DNS}), or
 %application of %\eqref{conv_T} and 
%Corollary \ref{cor:mod_of_cont}, % (or see already ),
%{\color{blue} \fbox{Propositions \ref{thm1} and \ref{prop:loc_conv} (??)}}
%Theorem \ref{thm_initial}, %\ref{thm::kr} and \ref{thm::dns_density}, 
%we know that there is some $\delta > 0$ %(with $(T,T + \delta) \subset \mathbb{T}^{(i)}$) 
%such that all $u \in [T,T+\delta]$ are continuity points of $\Lambda$ and, by Proposition \ref{pro::no_jump}, for any $\epsilon>0$ and $\Delta'$ small enough,
%	\begin{equation}\label{eqn:eps1}
%	\La_u - \La^{T, \Delta'}_u < \epsilon/3 %C_{p} \Delta^{p},
%	\end{equation}
%	for all such $u$. %$ \le T + \delta$. Fix this $\delta$. %, and now fix a value $\epsilon$. 
%Note that we must have $T + \delta < j$.
%	Fix a $\Delta'$ such that $T/\Delta'$ is an integer and that
%	\eqref{eqn:eps1} holds.
%	\[
%	C_{\varepsilon} (\Delta')^{\frac12 - \varepsilon} < \epsilon_3,
%	\]
%	for some $\epsilon_1$ to be chosen later. 
We now fix an $s\in(T,T+\teps]$. Then, $\lim_{\Delta\downarrow0} \lceil T/\Delta\rceil\Delta=T$, the right-continuity of $\Lambda$, and the preceding paragraph yield, for a sufficiently small $\overline{\Delta}\in(0,\overline{\Delta}_0)$,  
%We aim to show that we can find some $\Delta_*$, such that for all $\Delta < \Delta_*$, we have that
%	\begin{equation}
%	\label{lambda_spec}
%	\La_u - \La^\Delta_u < \epsilon,
%	\end{equation}
%	for all $u \in [T, T + \delta]$. %We start by using Theorem \ref{thm::kr} to find 
%By assumption, for all sufficiently small $\Delta''$ %there is a value $\Delta_*''$, such that for all $\Delta < \Delta_*'$, 
%we have 
\begin{equation}\label{Delta2}
\lceil T/\Delta\rceil\Delta\le s,\,
\Lambda_{\lceil T/\Delta\rceil\Delta}-\Lambda_T\le  \frac{\eta}{4C_\alpha(\overline{\Delta}_0\!-\!\overline{\Delta},\teps)}
\,\text{and}\,\La_T - \La^\Delta_T \le \frac{\eta}{4C_\alpha(\overline{\Delta}_0\!-\!\overline{\Delta},\teps)} ,\;\Delta\!\in\!(0,\overline{\Delta}],
\end{equation}
%for $u \in [0, T]$, 
%for some $\epsilon_2$ to be chosen later. 
where $C_\alpha(\overline{\Delta}_0-\overline{\Delta},\teps)\ge0$ is taken according to Corollary \ref{cor::discrete_compare} and is, in particular, non-increasing in the first argument.

\medskip

For any $\Delta\in(0,\overline{\Delta}]$ and integer multiple $\Delta_0\in[\overline{\Delta}_0-\overline{\Delta},\overline{\Delta}_0]$ of $\Delta$, we apply \eqref{Delta1}, followed by Corollary \ref{cor::discrete_compare} with $\CTT:=(0,\Delta,2\Delta,\ldots,\lceil T/\Delta\rceil\Delta,\lceil T/\Delta\rceil\Delta+\Delta_0,\lceil T/\Delta\rceil\Delta+2\Delta_0,\ldots)$
and \eqref{Delta2} to obtain
\begin{equation*}
\begin{split}
\La_s - \La^{\CTT}_s 
&= (\La_s - \La^{\lceil T/\Delta\rceil\Delta;\Delta_0}_s) 
+ (\La^{\lceil T/\Delta\rceil\Delta;\Delta_0}_s - \La^{\CTT}_s)  \\
&\le \frac{\eta}{2}+C_\alpha(\Delta_0,\teps)\cdot(\Lambda_{\lceil T/\Delta\rceil\Delta}-\La^\Delta_{\lceil T/\Delta\rceil\Delta}) \\
&\le\frac{\eta}{2}+C_\alpha(\overline{\Delta}_0-\overline{\Delta},\teps)\cdot\big((\Lambda_{\lceil T/\Delta\rceil\Delta}-\Lambda_T)+(\Lambda_T-\Lambda^\Delta_T)\big)\le\eta.
\end{split}
\end{equation*}
%	for $u \in [T, T + \delta]$. %with final term $T$. 	
%	Thus, for $\Delta < \Delta'_*$ such that $\Delta'/\Delta$ is an integer, we have that
%	\[
%	\La_u - \La^{(\Delta, 2\Delta, \dots, T, T+\Delta', \dots)}_{u} < C(T, T+\delta,\Delta') \epsilon_2 + \epsilon_1 %< \epsilon
%	\]
%	%for any $\epsilon>0$ 
%	for $\Delta$ small enough ($\Delta'$ fixed),
%	for all $u \in [T, T + \delta]$.	
Thus, $\Lambda_s-\Lambda^\Delta_s\le \eta$ by Remark \ref{rmk::discrete_general_prelim} and, since $\eta>0$ was arbitrary, $\lim_{\Delta\downarrow0} \Lambda^\Delta_s=\Lambda_s$. \ep
%, if we choose $\Delta' / \Delta''$ to be an integer, this implies
%	\begin{equation}\label{eq::before_jump_1}
%		\La_u - \La^{\Delta\!''}_u < 2 \epsilon/3.
%	\end{equation}
	%We can therefore first choose $\Delta'$ and then $\Delta$ accordingly such that \eqref{lambda_spec} is satisfied with $\Delta=\Delta''$, for given $\epsilon>0$ and all $u\in [T,T+\delta]$.



%We now fix an $s\in(T,T+\teps]$. Note that for any $\Delta>\Delta'>0$, it holds $\La^{\Delta}_{n\Delta} \ge \La^{\Delta'}_{n\Delta'}$, $n=0,\,1,\,\ldots\,$, by induction over $n$. 
%As $\La^{\Delta\!''}$  and $\La^{\Delta}$ are piecewise constant, we also have for all $u\ge 0$ that
%\begin{equation}\label{eq::before_jump_1aa}
%\La^{\Delta}_{u} \ge \La^{\Delta\!''}_{n\Delta\!''/\Delta}. 
%\end{equation}
%	because we have
%	\begin{equation}\label{eq::before_jump_2}
%		\La^{\Delta_2}_{n\Delta_2} = \widehat{\La}^{\Delta_1}_{n\Delta_1},
%	\end{equation}
%	where we define the process $( \widehat{X},  \widehat{\La})$ such that $ \widehat{X}_0 = \sqrt{\frac{\Delta_1}{\Delta_2}} X_0$, where we then note that $ \widehat{X}_0 > X_0$ and so $ \widehat{\La}^{\Delta_1} < \La^{\Delta_1}$ for all times. 
%	\chrb{\eqref{eq::before_jump_1a} ok also for non-integer multiples, as used below.}
%Further, since $\La$ is uniformly continuous in $[T, T + \delta]$, for any $\epsilon$ we may find some $\theta \in (0,1)$ such that for all $u \in [T, T + \delta]$ we have
%\begin{equation}\label{eq::before_jump_3}
%		\La_u - \La_{u (1 - \theta)} < \epsilon/3.
%	\end{equation}
%Thus, for any $\Delta\in(\Delta_0/M,\Delta_0/(M-1))$, we have
%\begin{equation*}
%\begin{split}
%\La_s - \La^{\Delta}_s \le \La_s - \La^{\Delta_0/M}_{\lfloor s/\Delta\rfloor\Delta_0/M} 
%=\big(\!\La_s-\La_{\lfloor s/\Delta\rfloor\Delta_0/M}\!\big)
%+\big(\!\La_{\lfloor s/\Delta\rfloor\Delta_0/M}-\La^{\Delta_0/M}_{\lfloor s/\Delta\rfloor\Delta_0/M}\!\big).
%\end{split}
%\end{equation*}
%For $M\in\mathbb{N}$ large enough, the first of the two parentheses is no larger than $\eta/2$ for all $\Delta\in(\Delta_0/M,\Delta_0/(M-1))$, thanks to 
%\begin{equation*}
%0\le s-\frac{\lfloor s/\Delta\rfloor\Delta_0}{M}\le s-\frac{(s(M-1)/\Delta_0-1)\Delta_0}{M}=\frac{s+\Delta_0}{M} 
%\end{equation*}
%and the uniform continuity of $\Lambda|_{[T,T+\teps]}$. The second parethesis is no larger than $\eta/2$ for all $\Delta\in(\Delta_0/M,\Delta_0/(M-1))$ and $M\in\mathbb{N}$ large enough, by the preceding paragraph and 
%\begin{equation*}
%s\ge \frac{\lfloor s/\Delta\rfloor\Delta_0}{M}\ge \frac{(s(M-1)/\Delta_0-1)\Delta_0}{M}=s-\frac{s+\Delta_0}{M}\ge T.
%\end{equation*}
%All in all, we have found for each $\eta>0$ and $s\in(T,T+\teps]$ an interval $(0,\overline{\Delta})$ such that $\Lambda_s-\Lambda_s^\Delta\le\eta$, $\Delta\in(0,\overline{\Delta})$. Thus, $\lim_{\Delta\downarrow0} \Lambda^\Delta_s=\Lambda^\Delta_s$, $s\in(T,T+\teps]$, as desired. \ep 

%by combining \eqref{eq::before_jump_1aa}, \eqref{eq::before_jump_3}, and \eqref{eq::before_jump_1}, in that order.
%We finish by choosing $\epsilon_2, \epsilon_1, $ and $\epsilon_3$ so that the right-hand side is at most $\epsilon$.
%Summarising the requirement on $\Delta$ as $\Delta'/n < \Delta < \Delta'/(n(1-\theta))$,
%	we can conclude by noting
%	that the union
%	\[
%	\bigcup_{n = m}^{\infty} \left( \frac{\Delta'}{n}, \frac{\Delta'}{n(1 - \theta)} \right)
%	\]
%	contains some set $(0, \Delta_*]$ for any $m$ and $\theta$.
%	{\color{blue}
%		%This is a contradiction to $s' = \inf ([0, j) \backslash \BTT)$ in the case $s'\in \BTT^{({\rm i})}$.
%		
%		%\textbf{Step 3: Extending past finitely many class (ii) points.}
%		
%		%The argument of Step 1 can still be applied to $s'=\inf \BTT^{({\rm ii})}$.
%		%Similarly, 
%		If now $s'\in \BTT^{({\rm ii})}$, then
%		there are $s_1 < s' < s_2$ such that $L_{s_2} - L_{s_1} < \epsilon / 2$, and by definition of $\BTT$, we may find some $\Delta_*$ such that 
%		\[
%		L_u - L^\Delta_u < \epsilon/2.
%		\]
%		for $\Delta < \Delta_*$ and $u \in [0, s_1]$. This choice of $\Delta_*$ suffices, because for any $u \in [s_1, s_2]$, we have that 
%		\[
%		L_u - L^\Delta_u \le L_{s_2} - L^\Delta_{s_1} = (L_{s_2}-L_{s_1}) + (L_{s_1}-L^\Delta_{s_1}) < \epsilon,
%		\]
%		as desired. Then, by an application of Corollary \ref{cor::discrete_compare}, analogous to above, we can extend convergence up to some $[s', s' + \delta)$.} \ep
%		%(in fact, the smaller of the next class (ii) point or $j$).
%		%,and by induction arbitrarily close to $j$ for any finite number of class (ii) points.

\subsection{Extension beyond discontinuity points} \label{sec::special_case}

The main result of this subsection is the following analogue of Proposition \ref{pro::no_jump} for the case that $T\ge0$ is a discontinuity point of $\Lambda$.
%As in the previous section, %Definition \ref{defTT}, 
%denote by $\mathbb{T}$ be the set of all $T\ge 0$ such that for any continuity point $t\in(0,T)$ of $\Lambda$ it holds $d_{\mathrm{M1}}\big(\Lambda^\Delta|_{[0,t]},\Lambda|_{[0,t]}\big)\underset{\Delta\downarrow0}{\longrightarrow}0$,
%and recall $\mathbb{T}^{\rm (iii)}$ from Theorem \ref{thm1}.

\begin{prop}\label{prop_jump}
%Let $T \in \mathbb{T} \cap \mathbb{T}^{\rm (iii)}$. 
Suppose Assumption \ref{ass}. Let $T\ge0$ be a discontinuity point of $\Lambda$ such that $\Lambda^\Delta|_{[0,t]}\underset{\Delta\downarrow0}{\overset{\emph{M1}}{\longrightarrow}}\Lambda|_{[0,t]}$ for any continuity point $t\in(0,T)$ of $\Lambda$. Then,  $\Lambda^\Delta|_{[0,T+\teps]}\underset{\Delta\downarrow0}{\overset{\emph{M1}}{\longrightarrow}}\Lambda|_{[0,T+\teps]}$ for all $\teps>0$ small enough.
%$T\ge0$ be a discontinuity point of $\Lambda$ such that for any continuity point $t\in(0,T)$ of $\Lambda$ it holds $d_{\mathrm{M1}}\big(\Lambda^\Delta|_{[0,t]},\Lambda|_{[0,t]}\big)\underset{\Delta\downarrow0}{\longrightarrow}0$. 
%Then, $d_{\mathrm{M1}}\big(\Lambda^\Delta|_{[0,T+\delta]},\Lambda|_{[0,T+\delta]}\big)\underset{\Delta\downarrow0}{\longrightarrow}0$ for some $\delta>0$.
\end{prop}

The proof of Proposition \ref{prop_jump} builds on two lemmas. The first investigates the cumulative distribution function of $X^{\Delta}_{T+\theta}$ on a right neighborhood of $0$, for small $\Delta$, $\theta$ and on the event $\inf_{0\le s<T+\theta} X^\Delta_s>0$, and provides an estimate akin to the one in Proposition \ref{thm1}(ii). 
%= X^{\CTT}_{t+d}$ 
%In particular, in order to attain a bound on the cumulative distribution function of $X^{\CTT}_{t+d}$. 
%We would essentially like to say that this quantity has density close to $1/\alpha$ for a right interval of 0 of appropriate size, so that if the continuous process is near ``explosion'', we can expect the same for the discrete process.
		
		
\begin{lem}\label{lem:jump-dens}
In the situation of Proposition \ref{prop_jump}, for any $\kappa>0$, there exist $\overline{\theta},\overline{\Delta}>0$ such that for all $\theta\in(0,\overline{\theta}]$ and all  $\Delta=(T+\theta)/1,\,(T+\theta)/2,\,\ldots\in(0,\overline{\Delta}]$,
\begin{equation}\label{eq::distrib_of_jump2}
\pp\Big(X^{\Delta}_{T + \theta} \le x,\,\inf_{0\le s<T+\theta} X_s^{\Delta} > 0\Big) \ge \frac{x-\kappa}{\alpha},\quad \kappa\le x\le\La_T - \La^{\Delta}_{T+\theta}. 
\end{equation}
\end{lem}

\noindent\textbf{Proof.}
		%Because $t \in \mathbb{T}^{\rm (iii)}$, by definition w
%		By the choice of $T$ as a discontinuity point we have %that $X_{t^-}$ satisfies 
%		by %Proposition \ref{thm1}
%		{\color{blue}\fbox{What best to cite?}}
By the minimality property \eqref{physical},
\[
\pp\Big( 0 < X_{T-} \le x,\,\inf_{0\le s<T} X_s > 0\Big) \ge \frac{x}{\alpha},\quad 	x \in [0, \La_T - \La_{T-}).
\]
%, by Definition \ref{defn::physical}. 
For any $\Delta>0$, we have $X_{T-}=X^\Delta_T+\Lambda^\Delta_T-\Lambda_{T-}$ (since $X_{T-}+\Lambda_{T-}=X_{0-}+B_T=X^\Delta_T+\Lambda^\Delta_T$) and $X^\Delta\ge X$, so  
\[
\pp\Big( 0 < X^\Delta_T+\Lambda^\Delta_T-\Lambda_{T-} \le x,\,\inf_{0\le s < T} X^{\Delta}_s > 0\Big) \ge \frac{x}{\alpha},
\quad x \in [0, \La_T - \La_{T-}).
\]
We use this assertion upon setting $\ell=\Lambda^\Delta_T-\Lambda_{T-}$ to obtain for all $y\in[-\ell,\La_T - \La_{T-}-\ell)$,
%\small
\begin{eqnarray}
&& \pp\Big(X^\Delta_T \le y,\,\inf_{0\le s <T} X^{\Delta}_s > 0 \Big) 
= \pp\Big( X^\Delta_T+\ell \le y+\ell,\,\inf_{0\le s < T} X^{\Delta}_s > 0 \Big) 
\ge \frac{y+\ell}{\alpha},\quad\mathrm{and\;thus} \nonumber \\
%&\ge \pp \Big( X^\Delta_T+\La^\Delta_T-\La_{T-} \le \min(y+\La^\Delta_T-\La_{T-},J)-\min(y+\La^\Delta_T-\La_{T-},0),\,\inf_{0\le s <T} X^{\Delta}_s > 0 \Big) \\
&&\pp\Big(X^\Delta_T \le y,\,\inf_{0\le s <T} X^{\Delta}_s > 0 \Big)\ge\frac{\min(y+\ell,\Lambda_T-\Lambda_{T-})-\min(y+\ell,0)}{\alpha}, \quad y\in\rr. 
\label{eq::distrib_of_jump} 
\end{eqnarray}

\smallskip

Next, we turn to $X^\Delta_{T+\theta}$, let $\widetilde{x}:=x+\La^{\Delta}_{T+\theta}-\Lambda_{T-}$, and observe 
%propagate by the increment of the Brownian motion, $W_{t + d} - W_t$. We have
\begin{equation*}
\begin{split}
&\pp\Big(X^{\Delta}_{T + \theta} \le x,\,\inf_{0\le s < T} X_s^{\Delta} > 0\Big) 
= \pp\Big( X^{\Delta}_T + B_{T+\theta} - B_T - \La^{\Delta}_{T+\theta} + \La^{\Delta}_{T} \le x,\,\inf_{0\le s < T} X_s^{\Delta} > 0 \Big) \\
&\qquad\qquad\qquad\quad\;\;\;
= \frac{1}{\sqrt{2\pi}} \int_{-\infty}^{\infty} e^{-\frac{z^2}{2}}\, 
\pp\Big(X^{\Delta}_T - \La^{\Delta}_{T+\theta} +  \La^{\Delta}_T  \le x + \sqrt{\theta}z,\,\inf_{0\le s < T} X_s^{\Delta} > 0 \Big)\,\mathrm{d}z \\
&\qquad\qquad\qquad\quad\;\;\;
\ge \frac{1}{\sqrt{2\pi}\alpha} \int_{-\infty}^{\infty} e^{-\frac{z^2}{2}}\,\big(\min(\widetilde{x}+\sqrt{\theta}z,\Lambda_T-\Lambda_{T-})-\min(\widetilde{x}+\sqrt{\theta}z,0)\big)\,\mathrm{d}z \\
&\qquad\qquad\qquad\quad\;\;\;
\ge \frac{1}{\sqrt{2\pi}\alpha} \int_{-\widetilde{x}/\sqrt{\theta}}^{(\Lambda_T-\Lambda_{T-}-\widetilde{x})/\sqrt{\theta}} e^{-\frac{z^2}{2}}\,
(\widetilde{x}+\sqrt{\theta}z)\,\mathrm{d}z,
\end{split}
\end{equation*}
where we have used  \eqref{eq::distrib_of_jump} to get the first inequality. 
%where we obtain the second line by the definition of $X^{\Delta}$, the third by integrating over the density of the increment of the Brownian motion, the fourth by using, and the last equation by dropping the integral where $x' + y\sqrt{d}/\alpha %\frac{y\sqrt{d}}{\alpha}> E$.
With Definition \ref{defn::discrete} and $(T+\theta)/\Delta\in\mathbb{N}$, 
\begin{equation*}
\pp\Big(X^{\Delta}_{T+\theta}\le x,\inf_{0\le s<T+\theta} X_s^{\Delta} > 0\Big) 
\ge\frac{1}{\sqrt{2\pi}\alpha} \int_{-\widetilde{x}/\sqrt{\theta}}^{(\Lambda_T-\Lambda_{T-}-\widetilde{x})/\sqrt{\theta}} 
\!\! e^{-\frac{z^2}{2}}(\widetilde{x}+\sqrt{\theta}z)\,\mathrm{d}z-\frac{\Lambda^\Delta_{T+\theta}\!
-\!\La^{\Delta}_{T-}}{\alpha}. 
\end{equation*}
Thus, given a $\kappa>0$, whenever $\theta>0$ is sufficiently small we have
\begin{equation}\label{numer_blowup}
\begin{split}
\pp\Big(X^\Delta_{T+\theta} \le x,\,\inf_{0\le s< T+\theta} X_s^{\Delta} > 0\Big) 
\ge \frac{x-\kappa/2}{\alpha}-\frac{\La_{T-} - \La^{\Delta}_{T-}}{\alpha},\\
\La_{T-} - \La^{\Delta}_{T+\theta}+\kappa/2\le x\le\La_T - \La^{\Delta}_{T+\theta}-\kappa,
\end{split}
\end{equation}
with the bounds on $x$ ensuring that the latter integration interval contains $[-\kappa/(2\sqrt{\theta}),\kappa/\sqrt{\theta}]$.  

\medskip		

We now claim that $\Lambda_{T-}-\Lambda^\Delta_{T-}\le\kappa/2$ for all $\Delta>0$ small enough. Indeed, this is obvious if $T=0$. For $T>0$, we let $t\in(0,T)$ be a continuity point of $\Lambda$ with the property $\Lambda_{T-}-\Lambda_t\le\kappa/4$. For all $\Delta>0$ small enough, $\Lambda_t-\Lambda^\Delta_t\le\kappa/4$, hence
\begin{equation*}
\Lambda_{T-}-\Lambda^\Delta_{T-}=(\Lambda_{T-}-\Lambda_t)+(\Lambda_t-\Lambda^\Delta_t)+(\Lambda^\Delta_t-\Lambda^\Delta_{T-})\le\frac{\kappa}{4}+\frac{\kappa}{4}+0=\frac{\kappa}{2}. 
\end{equation*}
In particular, $\La_{T-} - \La^{\Delta}_{T+\theta}\le\kappa/2$, and we deduce \eqref{eq::distrib_of_jump2} for $\kappa\le x\le\La_T - \La^{\Delta}_{T+\theta}-\kappa$ from \eqref{numer_blowup}.
%For every $\epsilon$, there is a continuity point $t'$ such that $\La_{T^-} - \La_{t'} < \epsilon/4$ and $T / (T - t') \in \mathbb{Z}$. By %Proposition \ref{pro::no_jump},
 %the assumptions on $T$,
%there is moreover some $\Delta$ such that $(T - t')/\Delta \in \mathbb{Z}$ and $\La_{t'} - \La^\Delta_{t'} < \epsilon/4$. Thus, we have found some $\Delta$ such that $T / \Delta \in \mathbb{Z}$ and $\La_{T^-} - \La^\Delta_T < \epsilon/2$, and %the conclusion 
%\eqref{eq::distrib_of_jump2}
%follows from \eqref{numer_blowup}
%for $\alpha x \in [\epsilon, \La_T - \La^{\Delta}_{T+d}-\epsilon]$. It trivially holds for $\alpha x < \epsilon$ and therefore it holds for $\alpha x \in [0, \La_T - \La^{\Delta}_{T+d}-\epsilon]$. 
For $\La_T - \La^{\Delta}_{T+\theta}-\kappa<x\le\La_T - \La^{\Delta}_{T+\theta}$, we use $\pp(X^{\Delta}_{T + \theta} \le x,\,\ldots\,) \ge \pp(X^{\Delta}_{T + \theta} \le x - \kappa,\,\ldots\,)$, apply \eqref{eq::distrib_of_jump2} with $x$ replaced by $x-\kappa$, and relabel $2\kappa$ as $\kappa$. \ep
%		Because we may choose $\Delta'$ such that $T/\Delta'$ is an integer,
%		% and $\La_{T^-} - \La^{\Delta'}_T$ is arbitrarily small ($\epsilon_2 + \epsilon_3$ from the beginning of the proof) 
%		by replacing $\Delta'$ with a divisor, we have that for each $\epsilon$, we can find $\Delta'$ and $d$ such that \eqref{eq::distrib_of_jump2} holds
%		for $\alpha x \in [\epsilon, \La_T - \La^{\Delta'}_{T+d})]$.
%		\begin{equation}\label{eq::distrib_of_jump2}
%			\BPP \left(X^{\Delta'}_{t + d} < \alpha x, \inf_{s \le t+d} X_s^{\Delta'} > 0\right) \ge x - \epsilon_5/\alpha,
%		\end{equation}
%		whenever $\alpha x \in [\epsilon_5, \La_t - \La^{\Delta'}_{t+d})]$. This is exactly what we wanted to show for the distribution of $\La^{\Delta'}_{t+d}$; that it is similar to the distribution of a process that would jump immediately at time $t+d$, and so that we suspect that we can now recover an instantaneous jump by setting $\Delta$ to be small.

\medskip

Next, we build on Lemma \ref{lem:jump-dens} to verify that the time-stepping scheme ``catches up'' with the physical solution. 

\begin{lem}\label{lem::special_case}
In the situation of Proposition \ref{prop_jump}, for any $\eta,\theta>0$, there exists some $\overline{\Delta}>0$ such that %$T/\Delta$ is an integer and  
%Let $t \in \mathbb{T} \cap \mathbb{T}^{\rm (iii)}$. 
$\La_T - \La^\Delta_{T+\theta}\le\eta$, $\Delta\in(0,\overline{\Delta}]$.
\end{lem}
	
\noindent\textbf{Proof.} We establish the lemma by proving the following statement: If, for some $\eta> 0$, it holds that for all $\theta>0$ we can find some $\overline{\Delta}>0$ such that %$T/\Delta$ is an integer and
$\La_T - \La^{\Delta}_{T+\theta} \le \eta$, $\Delta\in(0,\overline{\Delta}]$, then the same holds for $\frac23\eta$ in place of $\eta$.	
%As in the statement of Lemma \ref{lem::special_case}, 
To this end, we fix such an $\eta>0$ and any $\theta>0$. We seek a value of $\overline{\Delta}>0$ for which %$T/\Delta$ is an integer and 
$\La_T - \La^\Delta_{T+\theta} \le \frac23 \eta$, $\Delta\in(0,\overline{\Delta}]$. For any $\theta_0>0$, %(to be chosen later) and
the hypothesis of the statement yields a $\overline{\Delta}_0>0$ such that %$T/\widetilde{\Delta}$ is an integer and 
$\La_T - \La^{\Delta_0}_{T+\theta_0} \le \eta$, $\Delta_0\in(0,\overline{\Delta}_0]$. %Lemma \ref{lem::special_case}. 
By Lemma \ref{lem:jump-dens}, we may select $\theta_0$ and $\Delta_0$ to which \eqref{eq::distrib_of_jump2} also applies, with a $\kappa=\kappa(\eta,\theta)>0$ to be determined below. Our aim is to %will be to choose $\Delta$ such that $\Delta'/\Delta \in \mathbb{Z}$, and 
show that if $\theta_0$ is picked from a suitable interval $(0,\overline{\theta}_0]$, then $\widetilde{\Delta}>0$ can be chosen such that for all $\Delta=\Delta_0/1,\,\Delta_0/2,\,\ldots\in(0,\widetilde{\Delta}]$,  
%		$\La_T - \La^{\CTT}_{T+c} < \frac23 F$, where
%		\[
%		\CTT = (\Delta', 2\Delta', \dots, t, \dots, T+d, T+d + \Delta, T+d + 2\Delta, \dots).
%		\]
\begin{eqnarray}\label{taueqn}
\La_T - \La^{\CTT}_{T+\theta} \le \frac23 \eta,\;\text{with}\;
\CTT := (0,\Delta_0,2\Delta_0,\ldots, T+\theta_0,T+\theta_0+\Delta,T+\theta_0+2\Delta,\dots).
\end{eqnarray}
The claim then follows, since $\Lambda^\Delta_{T+\theta}\ge\La^{\CTT}_{T+\theta}$ by Remark \ref{rmk::discrete_general_prelim} (thus, $\Lambda_T-\Lambda^\Delta_{T+\theta}\le \frac23 \eta$) and the range $\bigcup_{\theta_0\in(0,\overline{\theta}_0]} \{(T+\theta_0)/1,(T+\theta_0)/2,\ldots\}\cap(0,\overline{\Delta}_0]$ of suitable $\Delta_0$ contains the interval $(0,\min(\overline{\theta}_0,\overline{\Delta}_0)]$ allowing us to take  $\overline{\Delta}=\min(\widetilde{\Delta},\overline{\theta}_0,\overline{\Delta}_0)>0$.  

\medskip
		
Fix any $\Delta=\Delta_0/1,\,\Delta_0/2,\,\ldots$ and
%and start taking steps of size $\Delta$ after reaching time $t+d$; that is, we consider $\La^{\CTT}_{t + d + n\Delta}$ for
%\[
%\CTT = (\Delta', 2\Delta', \dots, t+d, t+d + \Delta, t+d + 2\Delta, \dots).
%\]
let $\ell_n:=\La^{\CTT}_{T+\theta_0+n\Delta}-\La^{\Delta_0}_{T+\theta_0}$, $n=0,\,1,\,\ldots\,$. 
%the amount of loss past time $j+d$, 
%which implicitly depends first on our choice of $d$ and $\Delta'$ such that \eqref{eq::distrib_of_jump2} holds, and then on our choice of $\Delta$.
Then,
\[
\begin{split}
\ell_{n+1} &= \alpha\pp\Big(\inf_{0\le s<T+\theta_0} X_s^{\Delta_0} > 0,\,\min_{0\le m \le n} X^{\CTT}_{T +\theta_0+m\Delta} < 0\Big) \\
& \ge 
\alpha\pp\Big(\inf_{0\le s<T+\theta_0} X_s^{\Delta_0} > 0,\,X^{\CTT}_{T+\theta_0+n\Delta} < 0\Big) \\
& = \frac{\alpha}{\sqrt{2\pi}} \int_{-\infty}^{\infty} e^{-\frac{z^2}{2}}\,
\pp\Big(\inf_{0\le s<T+\theta_0} X_s^{\Delta_0} > 0,\,X^{\Delta_0}_{T+\theta_0} < \sqrt{n\Delta} z + \ell_n \Big)\,\mathrm{d}z.
\end{split}
\]
%where we may integrate over the density of the increment $B_{j+d+n\Delta} - B_{j+d}$,
Next, we set $\widetilde{\ell}=\Lambda_T-\Lambda^{\Delta_0}_{T+\theta_0}$ and apply %the bound we attained about the distribution of $Y^{\Delta'}_{j+d}$, Equation 
\eqref{eq::distrib_of_jump2} in the form
\[
\pp\Big(X^{\Delta_0}_{T+\theta_0} < x,\,\inf_{0\le s<T+\theta_0} X_s^{\Delta_0} > 0\Big) 
\ge\frac{\min(x-\kappa,\widetilde{\ell}-\kappa)-\min(x-\kappa,0)}{\alpha},\quad x\in\rr
\]
to obtain the explicit recursive inequality 
\[
\ell_{n+1}\ge\frac{1}{\sqrt{2\pi}} \int_{-\infty}^{\infty} e^{-\frac{z^2}{2}}\,
\Big(\!\min\big(\sqrt{n\Delta}z + \ell_n - \kappa,\widetilde{\ell}-\kappa\big) 
- \min\big(\sqrt{n\Delta}z + \ell_n - \kappa,0\big)\!\Big)\,\mathrm{d}z.
\]
% FIX THIS EVENTUALLY, INTRODUCE f FIRST, THEN DON'T DO BIG EXPANSIONS
% this is probably fine actually
We rewrite the latter using the standard Gaussian cumulative distribution function $\Phi$:
\[
%		M_{n+1} &\ge&
\ell_{n+1}\ge\frac{1}{\sqrt{2\pi}} \int_{(\kappa-\ell_n)/\sqrt{n\Delta}}^{(\widetilde{\ell} - \ell_n)/\sqrt{n\Delta}}  e^{-\frac{z^2}{2}}\,\big(\sqrt{n\Delta}z+\ell_n-\kappa\big)\,\mathrm{d}z 
		 %\\ &&
		 + (\widetilde{\ell}-\kappa)\bigg(1-\Phi \bigg(\frac{\widetilde{\ell}-\ell_n}{\sqrt{n\Delta}}\bigg)\!\bigg).
%		  \\
%		&=& (M_n - \epsilon_5) \left( \Phi\left( \frac{\alpha(F'-M_n)}{\sqrt{n\Delta}} \right) - \Phi\left(- \frac{\alpha(M_n-\epsilon_5)}{\sqrt{n\Delta}} \right)\right) \\
%		&& -\frac{\sqrt{n\Delta}}{\alpha \sqrt{2\pi}}\left( \exp\left(-\frac{\alpha^2(F' - M_n)^2}{2n\Delta} \right) - \exp\left(-\frac{\alpha^2(M_n - \epsilon_5)^2}{2n\Delta} \right)\right)
%		+ (F' - \epsilon_5)\left( 1 - \Phi \left( \frac{\alpha(F'-M_n)}{\sqrt{n\Delta}} \right)\right).
\]
Integrating by parts and introducing 
\[
f(x):=\int_{-\infty}^x \Phi(z)\,\mathrm{d}z=x\Phi(x) + \frac{1}{\sqrt{2\pi}}\,e^{-\frac{x^2}{2}},\quad x\in\rr
\]
we further deduce 
\[
\ell_{n+1} \ge \widetilde{\ell} - \kappa - \sqrt{n\Delta}\,\bigg(f\bigg(\frac{\widetilde{\ell}-\ell_n}{\sqrt{n\Delta}} \bigg) - f\bigg(\frac{\kappa-\ell_n}{\sqrt{n\Delta}} \bigg)\!\bigg).
\]
In view of $\Phi(x)+\Phi(-x)=1$, $x\in\rr$, we have $f(x)=f(-x)+x$, $x\in\rr$, so 
\[
\ell_{n+1} \ge \ell_n - \kappa + \sqrt{n\Delta}\,\bigg(f\bigg(\frac{\kappa-\ell_n}{\sqrt{n\Delta}}\bigg) 
-f\bigg(\!-\frac{\widetilde{\ell}-\ell_n}{\sqrt{n\Delta}}\bigg)\!\bigg).
\]
Since $f'=\Phi$ is increasing, we arrive at
\begin{equation}\label{eq::jump_recursion}
\ell_{n+1} \ge \ell_n - \kappa + \Phi\bigg(\!-\frac{\widetilde{\ell}-\ell_n}{\sqrt{n\Delta}} \bigg)
\cdot(\kappa-2\ell_n+\widetilde{\ell}),
\end{equation}
provided that $\kappa-2\ell_n+\widetilde{\ell}\ge 0$.
		
		%We now conclude to deduce \eqref{taueqn}.
%		Recall that we may choose some $\epsilon_5$ and $d$, we can find a step size $\Delta'$ such that $\La_t - \La^{\Delta'}_{t+d} < F$ and such that \eqref{eq::distrib_of_jump2} holds; our objective is to find a further step size $\Delta$ such that $\Delta'/\Delta \in \mathbb{Z}$ and such that $\La_t - \La^{\CTT}_{t+d+n\Delta} < \frac23 F$, where we require that $d + n\Delta < c$, and we define $\CTT = (\Delta', 2\Delta', \dots, t+d, t+d + \Delta, t+d + 2\Delta, \dots)$. We need only that $d < c$ and our choice of $\epsilon_5$ will come later.		
		%Say that we have the step size $\Delta'$ for our choice of $\epsilon$ and $d$. 

\medskip

To prove \eqref{taueqn}, and thus the lemma, we assume $\widetilde{\ell}>2\eta/3$ (otherwise \eqref{taueqn} holds with $\theta_0=\theta$ and $\widetilde{\Delta}=\overline{\Delta}_0$) and show that if $\theta_0\in(0,\theta)$ is taken small enough and the integers $(T+\theta_0)/\Delta_0$ and $\Delta_0/\Delta$ are made large enough, then one 
can find an $n\ge0$ with $\theta_0+n\Delta\le\theta$ and $\widetilde{\ell}/3\le \ell_n$. The inequality $\La_T - \La^{\CTT}_{T+\theta} \le  2\eta/3$ in \eqref{taueqn} then follows from 
\[
\La_T-\La^{\CTT}_{T+\theta_0+n\Delta}
=(\La_T-\La^{\Delta_0}_{T+\theta_0})+(\La^{\Delta_0}_{T+\theta_0}-\La^{\CTT}_{T+\theta_0+n\Delta})
\le \frac{2(\La_T-\La^{\Delta_0}_{T+\theta_0})}{3}\le\frac{2\eta}{3}.
\]
%Summarizing, for any $\eta>0$, we can choose $\theta_0\in(0,\theta)$ sufficiently small and $\Delta_0>0$ such that \in \mathbb{Z}$, $\widetilde{\ell}=\La_T - \La^{\Delta_0}_{T+\theta_0} \le \eta$, and \eqref{eq::jump_recursion} holds.  it then suffices to find some $\Delta>0$ for which $n\Delta < \theta - \theta_0$ and $\frac13 \widetilde{\ell} \le \ell_n$, 
%\[
%\frac13 \widetilde{\ell} \le \ell_n \;\; \Leftrightarrow   \;\;
%\frac13 (\La_T - \La^{\Delta_0}_{T+\theta_0}) \le  \La^{\CTT}_{T + \theta_0 + n\Delta} - \La^{\Delta_0}_{T+\theta_0}  \;\; \Leftrightarrow  \;\;
%\La_T - \La^{\CTT}_{T + \theta_0 + n\Delta} \le \frac23 \widetilde{\ell} < \frac23 \eta.
%\]
%noting that $F' = \La_t - \La^{\Delta'}_{t+d} < F$ by the assumption made on the outset. 
Arguing by contradiction, suppose that $\ell_n<\widetilde{\ell}/3$ for all $n=0,\,1,\,\ldots,\,\lfloor(\theta - \theta_0)/\Delta\rfloor=:n_0$. Summing \eqref{eq::jump_recursion} over $0\le n\le n_0-1$ upon noting that $\kappa-2\ell_n+\widetilde{\ell}>\kappa+\widetilde{\ell}/3>\kappa+\ell_0=\kappa>0$ for such $n$ we get
\begin{eqnarray*}
\ell_{n_0} \ge -\kappa n_0 + \sum_{n = 0}^{n_0-1} \Phi\bigg(\!- \frac{\widetilde{\ell}-\ell_n}{\sqrt{n\Delta}}\bigg)
\cdot(\kappa-2\ell_n+\widetilde{\ell}).
\end{eqnarray*}
Using $\kappa-2\ell_n+\widetilde{\ell}>\widetilde{\ell}/3$ and $\widetilde{\ell}-\ell_n\le\widetilde{\ell}$ we deduce 
\[
\begin{split}
\ell_{n_0} 
\ge -\kappa n_0 
+\frac{\widetilde{\ell}}{3}\,\sum_{n = 0}^{n_0-1} \Phi\bigg(\!-\frac{\widetilde{\ell}}{\sqrt{n\Delta}} \bigg) 
&\ge n_0\bigg(\!-\kappa+\frac{\widetilde{\ell}}{6}\, \Phi\bigg(\!-\frac{\sqrt2\widetilde{\ell}}{\sqrt{\theta-\theta_0-2\Delta}} \bigg)\!\bigg) \\
&\ge n_0\bigg(\!-\kappa+\frac{\eta}{9}\, \Phi\bigg(\!-\frac{\sqrt2\eta}{\sqrt{\theta-\theta_0-2\Delta}} \bigg)\!\bigg),
\end{split}
\]
where we have dropped the summands with $n<n_0-\lceil n_0/2\rceil$ and have employed a common lower bound for the remaining summands. We choose $\kappa=\kappa(\eta,\theta)>0$ such that the latter bracket is positive, observing that the smaller $\theta_0+2\Delta>0$ is, the larger this bracket becomes. Lastly, we pick $\Delta>0$ dividing $\Delta_0$ so that $n_0$ is large and the final lower bound on $\ell_{n_0}$ is at least $\Lambda_T/3\ge\widetilde{\ell}/3$, giving us the desired contradiction. The proof is complete. \ep
		
\medskip	
%\begin{lemma}\label{thm::special_case}
%	%Let $(X, \La)$ satisfy \eqref{eq::init1} and \eqref{eq::init2}, % for some initial condition $Y_0$ and parameter $\alpha$, such that the hypotheses of 
%	%Theorem \ref{thm::main} hold. 
%	%and let $j \in \mathbb{T}^{\rm (iii)}$. % be the first time at which $Y$ and $L$ are discontinuous. 
%	Let $t \in \mathbb{T} \cap \mathbb{T}^{\rm (iii)}$. 
%	Then, for all $\epsilon > 0$, for sufficiently small $\Delta$, there is $s > t$ such that $\La_s - \La^\Delta_s < \epsilon$ and $s - t < \epsilon$.
%\end{lemma}
%
%\begin{proof}
%
%	As in Proposition \ref{pro::no_jump}, we first show that there is some $\Delta$ such that the above statement holds, and we use the same procedure as the end of the proof of Proposition \ref{pro::no_jump} to deduce the same result for sufficiently small $\Delta$.
%		
%%Let $L_j - L_{j^-} = E$. 
%%		We first note that this lemma proves the theorem. 
%%		The initial hypotheses for the lemma are true for $F = E + \epsilon_2 + \epsilon_3$, and hence they are true for $F = \epsilon_4$, for any $\epsilon_4$, by repeatedly applying the lemma. 
%%		In particular, 
%By Lemma \ref{lem::special_case},
%		we can choose $\epsilon_5$ and find a $\Delta$ such that $t/\Delta \in \mathbb{Z}$ and $\La_t - \La^\Delta_{t+\epsilon_5}  < \epsilon_4$. Now, choose $\epsilon_5$ such that $\epsilon_5 < \epsilon$ and such that $\La_{t + \epsilon_5} - \La_t < \epsilon_6$ for some $\epsilon_6$, which is always possible because $\La$ is continuous in that region. Finally, choose $\epsilon_4$ and $\epsilon_6$ such that $\epsilon_4 + \epsilon_6 < \epsilon$, and we have found one value $\Delta$ such that $\La_s - \La^\Delta_s < \epsilon$ for some $s$ such that $s - t < \epsilon$.
%	
%%	To extend this to all sufficiently small $\Delta$, we apply the same arguments in the final part of the proof of Proposition \ref{pro::no_jump}. We will provide the details after proving Lemma \ref{lem::special_case}.
%	
%%	To finish the proof of Lemma \ref{thm::special_case}, w
%%	We now note that by the discussion before the proof of Lemma \ref{lem::special_case}, by repeating Lemma \ref{lem::special_case}, we may get one value $\Delta$ for which $L_k - L^\Delta_k < \epsilon_2$ for some $k$ such that $k - j < \epsilon_2$. 
%	We now wish to prove that there is some step size $\Delta_*$ such that for all $\Delta' < \Delta_*$, we have $\La_s - \La^{\Delta'}_s < \epsilon$ for some $s$ such that $s - t < \epsilon$. We note that by the continuity of $\La$ immediately after $t$, % and assuming that the discontinuities of $L$ have no accumulation points, 
%	for all $\epsilon_4$, we can find $\epsilon_3$ such that $\La$ is continuous on $[s, s + \epsilon_3]$ and $\La_{s + \epsilon_3} - \La_s < \epsilon_4$.
%	Hence, analogous to the proof of  Proposition \ref{pro::no_jump}, for every integer $n$ and for every $\Delta'$ satisfying
%	\[
%	\frac{\Delta}{n} < \Delta' < \frac{\Delta}{n} \frac{s + \epsilon_3}{s},
%	\]
%	we have that $\La_{s + \epsilon_3} - \La^{\Delta'}_{s + \epsilon_3} < \epsilon_2 + \epsilon_4$. Choose $\epsilon_4$ and $\epsilon_3$ such that $\epsilon_2 + \epsilon_4 < \epsilon$ and $\epsilon_2 + \epsilon_3 < \epsilon$, and note that union the above constraints for $\Delta'$ contains an interval $[0, \Delta_*]$ to conclude.	
%%	This concludes the proof of Lemma \ref{thm::special_case}.
%\end{proof}
%
%
%
%
%\noindent\textbf{Proof.}
We are now ready to show Proposition \ref{prop_jump}.

\medskip

\noindent\textbf{Proof of Proposition \ref{prop_jump}.} We start by using Propositions \ref{thm1} and \ref{prop:density_est}(a) to find an $\teps>0$ such that \eqref{loc_rate_conv} applies to all $T\le t\le T+\teps$ with this $\teps$. In particular, upon fixing $s\in(T,T+\teps]$ and $\eta>0$ we can select some $\overline{\Delta}_0>0$ so that
\begin{equation}\label{eta/2bnd}
\Lambda_s-\Lambda^{t;\Delta_0}_s\le\frac{\eta}{2},\quad t\in[T,s],\quad\Delta_0\in(0,\overline{\Delta}_0]. 
\end{equation}
Next, we recall the quantity $C_\alpha(\overline{\Delta}_0/2,s-T)\ge0$ from Corollary \ref{cor::discrete_compare} and choose $\theta_0\in(0,s-T]$ with the property
\begin{equation}\label{rightcont}
\Lambda_{T+\theta_0}-\Lambda_T\le\frac{\eta}{4C_\alpha(\overline{\Delta}_0/2,s-T)}. 
\end{equation} 
Finally, we rely on Lemma \ref{lem::special_case} to pick $\widetilde{\Delta}>0$ so that 
\begin{equation}\label{catchup}
\Lambda_T-\Lambda^\Delta_{T+\theta_0/2}\le\frac{\eta}{4C_\alpha(\overline{\Delta}_0/2,s-T)},\quad\Delta\in(0,\widetilde{\Delta}]. 
\end{equation}
Then, for $\Delta\in(0,\min(\widetilde{\Delta},\overline{\Delta}_0/2,\theta_0/2)]$ and $\Delta_0\in[\overline{\Delta}_0/2,\overline{\Delta}_0]$ such that $\Delta_0/\Delta$ is an integer, we get with $t=\lfloor (T+\theta_0)/\Delta\rfloor\Delta\in[T+\theta_0/2,T+\theta_0]$ and $\CTT=(0,\Delta,2\Delta,\ldots,t,t+\Delta_0,t+2\Delta_0,\ldots)$, 
\begin{equation}
\begin{split}
\Lambda_s-\Lambda^\Delta_s\le \Lambda_s-\Lambda^{\CTT}_s
&=(\Lambda_s-\Lambda^{t;\Delta_0}_s)+(\Lambda^{t;\Delta_0}_s-\Lambda^{\CTT}_s) \\
&\le\frac{\eta}{2}+C_\alpha(\overline{\Delta}_0/2,s-T)(\Lambda^{t;\Delta_0}_t-\Lambda^{\CTT}_t) \\
&=\frac{\eta}{2}+C_\alpha(\overline{\Delta}_0/2,s-T)\big((\Lambda_t-\Lambda_T)
+(\Lambda_T-\Lambda^\Delta_t)\big)\le\eta,
\end{split}
\end{equation}
where we have used Remark \ref{rmk::discrete_general_prelim}, \eqref{eta/2bnd}, Corollary \ref{cor::discrete_compare}, Definition \ref{defn::discrete_general}, \eqref{rightcont}, and \eqref{catchup} in this order. 
Since $s\in(T,T+\teps]$ and $\eta>0$ were arbitrary, we conclude that $\lim_{\Delta\downarrow0} \Lambda^\Delta_s=\Lambda_s$, $s\in(T,T+\teps]$, thus obtaining the proposition. \ep

%We first show that for all $\epsilon > 0$, there is $s > t$ and $\Delta$ such that $t/\Delta \in \mathbb{Z}$, $\La_s - \La^\Delta_s < \epsilon$ and $s - t < \epsilon$. By Lemma \ref{lem::special_case}, for all $\epsilon>0$
%		and $0<\delta<\epsilon$ we can choose $\Delta$ such that $T/\Delta \in \mathbb{Z}$ and $\La_T - \La^\Delta{T+\delta}  < \epsilon/2$. Now choose 
%$\delta$ such that $\delta < \epsilon$ and 
%		$\delta$ such that $\La_{T + \delta} - \La_T < \epsilon/2$, which is always possible because $\La$ is continuous in that region,
%Finally, choose $\epsilon_4$ and $\epsilon_6$ such that $\epsilon_4 + \epsilon_6 < \epsilon$, and 
%		and we have found one value of $\Delta$ such that $\La_s - \La^\Delta_s < \epsilon$ for some $s$ such that $s - T < \epsilon$.

%We can now use the same procedure as at the end of the proof of Proposition \ref{pro::no_jump} to deduce the same result for sufficiently small $\Delta$ (and not only a specific $\Delta$ as chosen above).
%We therefore have that for all $\varepsilon>0$ there exists some $T'=T'(\varepsilon)\in(T,T+\varepsilon]$ and $\Delta_*=\Delta_*(\varepsilon)>0$ such that for all $\Delta\in(0,\Delta_*]$ it holds $\Lambda_{T'}-\Lambda^\Delta_{T'}\le\varepsilon$. 

%To show the proposition, pick any $\delta>0$ so that 
%$(T,T+\delta]$ %(recall Theorem \ref{thm1}). 
%contains only continuity points of $\Lambda$.
%Then, for any $r,\varepsilon\in[0,\delta]$ 
%and all $\Delta\in(0,\Delta_*(\varepsilon)\!)$ and positive integer multiples $\Delta'$ of $\Delta$,
%we have with $\CTT:=(0,\,\Delta,\,2\Delta,\,\ldots,\,T',\,T'+\Delta',\,T'+2\Delta',\,\ldots)$ by Corollary \ref{cor::discrete_compare} (recall also Remark \ref{rmk::discrete_general_prelim} and the notation introduced in Definition \ref{defn::discrete_general}: % \ref{defn::continuous_then_discrete}):
%\begin{equation}\label{prop2split}
%\begin{split}
%\Lambda_{T+r}-\Lambda^\Delta_{T+r} \le \Lambda_{T+r}-\Lambda^{\CTT}_{T+r}
%= \big(\Lambda_{T+r}\!-\!\Lambda_{T+r}^{T',\Delta'}\big)
%+\big(\Lambda_{T+r}^{T',\Delta'}\!-\!\Lambda^{\CTT}_{T+r}\big) \qquad\qquad\qquad\qquad\quad\;\; \\
%\le \big(\Lambda_{T+r}\!-\!\Lambda_{T+r}^{T',\Delta'}\big) 
%+ C\big(\Lambda_{T'}\!-\!\Lambda^\Delta_{T'}\big) 
%\le\big(\Lambda_{T+r}\!-\!\Lambda_{T+r}^{T',\Delta'}\big) + C\varepsilon,
%\end{split}
%\end{equation}
%where $T'=T'(\varepsilon)\in(T,T+\varepsilon]$ and $C=C(\Delta',T',T+r)$. Since 
%\begin{eqnarray*}
%&& \Lambda_{T+r}-\Lambda_{T'}= (\alpha-\Lambda_{T'})\,\pp\Big(\min_{t\in[T',T+r]} X_t \le 0\,\Big|\,\min_{t\in[0,T']} X_t>0\Big), \\
%&& \Lambda_{T+r}^{T',\Delta'}-\Lambda_{T'}^{T',\Delta'}= (\alpha-\Lambda_{T'})\,\pp\Big(\min_{0\le m\le \lfloor (T+r-T')/\Delta'\rfloor-1} X^{T',\Delta'}_{T'+m\Delta'} \le 0\,\Big|\,\min_{t\in[0,T']} X_t>0\Big),
%\end{eqnarray*}
%Proposition \ref{prop:loc_conv}, applied under the conditional measure $\pp(\,\cdot\,|\min_{t\in[0,T']} X_t>0)$, reveals
%\footnote{\textcolor{magenta}{Choice of $\delta$ depends on how Theorem \ref{thm::kr} is phrased eventually.}}
%that the term $\Lambda_{T+r}\!-\!\Lambda_{T+r}^{T',\Delta'}$ in \eqref{prop2split}
%can be made arbitrarily small by choosing $\Delta'$ in a suitable range $(0,\Delta'_*]$, and the proposition follows. \ep
%\textbf{TO DO: conclusion.} Thus, Proposition \ref{prop_jump} is a consequence of Lemma \ref{thm::special_case}. 
%\ep

%{\color{blue} \fbox{Perhaps best to first prove the following theorem in the setting of Proposition \ref{pro::no_jump},}\\
%	\fbox{i.e.\ starting from the regular regime, and then bring together to allow a ``jump start''. }}
\subsection{Proof of Theorem \ref{thm::main}} \label{sec::post_jump}

Theorem \ref{thm::main} follows directly from Propositions \ref{pro::no_jump}~and~\ref{prop_jump}. Indeed, we can argue by contradiction and assume the existence of continuity points $s\in(0,\infty)$ of $\Lambda$ for which the convergence $\Lambda^\Delta|_{[0,s]}\underset{\Delta\downarrow0}{\overset{\text{M1}}{\longrightarrow}}\Lambda|_{[0,s]}$ does not hold. Let $T\ge0$ be the infimum of such continuity points. If $T$ is a continuity point of $\Lambda$, we rely on Proposition~\ref{pro::no_jump} to infer $\Lambda^\Delta|_{[0,T+\teps]}\underset{\Delta\downarrow0}{\overset{\text{M1}}{\longrightarrow}}\Lambda|_{[0,T+\teps]}$ for all $\teps\ge0$ small enough. If $T$ is a discontinuity point of~$\Lambda$, we apply Proposition \ref{prop_jump} to get $\Lambda^\Delta|_{[0,T+\teps]}\underset{\Delta\downarrow0}{\overset{\text{M1}}{\longrightarrow}}\Lambda|_{[0,T+\teps]}$ for all $\teps>0$ small enough. This contradiction to the definition of $T$ yields the theorem. \ep 

\begin{rmk}
It is worth noting that the proof of Theorem \ref{thm::main} remains intact if instead of Assumption \ref{ass}(a), the boundedness of $f$ on $[0,\infty)$ together with the conclusions of Lemma~\ref{lemma:a priori} and Corollary \ref{cor:mod_of_cont} are assumed and $\psi:=\Psi':\,(0,\delta]\to\big(0,\frac{1}{\alpha}\big]$ is a strictly increasing function. Indeed, the proof of Theorem \ref{thm::main} can be then repeated word by word, and \eqref{loc_rate_conv}, used in the proofs of Propositions \ref{pro::no_jump} and \ref{prop_jump}, can be obtained via Remark \ref{alt_ass}. 
\end{rmk}


%Assume the contrary, i.e., there exist continuity points where 
%$\Lambda^\Delta|_{[0,T]}\underset{\Delta\downarrow0}{\cancel{\longrightarrow}}\Lambda|_{[0,T]}$ in $(D([0,T]),d_{\mathrm{M1}})$.
%$\Lambda^\Delta|_{[0,T]} \nrightarrow \Lambda|_{[0,T]}$ in $(D([0,T]),d_{\mathrm{M1}})$ as $\Delta\downarrow0$.
%$\La^\Delta$ does \emph{not} converge. 
%Let $0\le T'<\infty$ be the infimum of all such points.
%Then, if $T'$ is a continuity point or discontinuity point, by Propositions \ref{pro::no_jump} and \ref{prop_jump}, respectively, we have that
%$\Lambda^\Delta|_{[0,T'+\delta]}\underset{\Delta\downarrow0}{\longrightarrow}\Lambda|_{[0,T'+\delta]}$ in the M1 sense, for some $\delta>0$.

%{\color{blue} \fbox{Add concrete reference for the following `fact'.}}
%From this it follows directly \chrb{check this is true -- argument may depend on definition of metric}
%Using the fact that for monotone functions $d_{\mathrm{M1}}$-convergence is equivalent to pointwise convergence at all continuity points,
%it follows directly that $\Lambda^\Delta|_{[0,T]}\underset{\Delta\downarrow0}{\longrightarrow}\Lambda|_{[0,T]}$ in $(D([0,T]),d_{\mathrm{M1}})$ for all continuity points $T \in [0,T'+\delta)$, leading to a contradiction. Hence Theorem \ref{thm::main} holds.





 


==> arXiv v2/Section5_final.tex <==
%!TEX root =Main.tex

\section{Numerical simulations}  \label{sec::numerical}

In this last section, we examine the convergence of the time-stepping scheme (recall Definition \ref{defn::discrete}) numerically, for various initial densities $f$ and resulting functions $\Lambda$ with and without discontinuities. We write $L^\Delta$ for $\Lambda^\Delta/\alpha$, so that $L^\Delta_{n\Delta}
= \pp\big(\!\min_{0\le m\le n-1} X_{m\Delta}^\Delta<0\big)$, $n=1,\,2,\,\ldots\,$, % as in \cite{KR}, 
and simulate the latter probabilities by a Monte Carlo particle method with $N=10^7$ particles, following \cite[Algorithm 1]{KR}. This fully implementable scheme
is given for completeness in the appendix, where we also derive the convergence as $N\rightarrow \infty$.
This extends the convergence result from \cite{KR}, which is restricted to the regular case studied there, and additionally shows the order $O(1/\sqrt{N})$ for fixed $\Delta$.
 
%\subsection{Skorokhod M1 distance between two piecewise constant functions} 
%
%We first summarize the algorithm introduced in \cite[Section 2.3]{deshmukh2017quantifying} to compute the Skorokhod M1 distance between two piecewise constant functions, which we apply to our numerical solutions below. 
%
%\medskip
%
%Consider a sequence $0 = t_0 < t_1 < \cdots < t_n = T$ and two functions $g,\,h:\,[0, T] \rightarrow \mathbb{R}$ such that $g(t)=g_i$ for $t_{i-1}\le t<t_i$ and $h(t)=h_i$ for $t_{i-1}\le t<t_i$, $i=1,\,2,\,\ldots,\,n$. We seek to compute the Skorokhod M1 distance $d_{\mathrm{M1}}(g,h)$, defined by %Section \ref{sec:prelim}, Definition \ref{defn::m1} 
%\begin{equation*}
%d_{\mathrm{M1}}(g,h) = \min_{\lambda(\cdot) \in \Omega} \max\Big(\sup_{t \in [0, T]} | \lambda(t) - t |, \sup_{t \in [0, T]} |g(\lambda(t)) - h(t)|\Big),
%\end{equation*}
%where $\Omega$ is a class of strictly increasing continuous mappings of $[0, T]$ on itself.
%
%\medskip
%
%We consider the following set of points $\{t_0,  t_1^{-}, t_1, t_2^{-}, t_2, 
%\ldots, t_n^{-}, t_n \}$,  where $t_i^{-} = t_i - \epsilon$ for small $\epsilon>0$, a point that is very close to $t_i$ from the left. It is clear that $f(t_i) = f_i$ and $f(t_i^{-}) = f_{i-1}$,
%and similar for $g$. % The same hold for $g$: $g(t_i) = g_i$ and $g(t_i^{-}) = g_{i-1}$. 
%For convenience of notation, in the following we use 
%\begin{align*}
%	\{\tilde{t}_0, \tilde{t}_1, \ldots, \tilde{t}_{2n} \} &= \{t_0,  t_1^{-}, t_1, t_2^{-}, t_2, 
%\ldots, t_n^{-}, t_n \}, \\
%	\{\tilde{f}_0,\tilde{f} _1, \ldots, \tilde{f}_{2n} \} &= \{f_0,  f_0, f_1, f_1, f_2, f_2 
%\ldots, f_{n-1}, f_{n-1}, f_n \}, \\
%	\{\tilde{g}_0,\tilde{g} _1, \ldots, \tilde{g}_{2n} \} &= \{g_0,  g_0, g_1, g_1, g_2, g_2 
%\ldots, g_{n-1}, g_{n-1}, g_n \}.
%\end{align*}
%%To find the Skorokhod distance, a 
%A dynamic programming-type algorithm in \cite[Section 2.3]{deshmukh2017quantifying}
%%. Let $M(i, j)$ the Skorokhod distance up to $\tilde{t}_i$ when the point $\tilde{t}_j$ has been moved to match the point $\tilde{t}_i$. Hence, it is not difficult 
%gives a recurrent formula for a quantity $M(i, j)$,
%%\begin{equation}
%%	M(i, j) = \min \left( \begin{aligned} 
%%									&\max(M(i-1, j-1), d(\tilde{f}_i, \tilde{g}_j)) \\
%%									&\max(M(i, j-1), d(\tilde{f}_i, \tilde{g}_j)) \\
%%									&\max(M(i-1, j), d(\tilde{f}_i, \tilde{g}_j))
%%								\end{aligned}
%%						\right),
%%\end{equation}
%\begin{equation}
%	M(i, j) = \max\left(\min\left(M(i-1, j-1), M(i, j-1), M(i-1, j)\right), |t_i - t_j|, |f_i - g_j|\right)),
%\end{equation}
%with the initial condition $M(0, 0) = |f_0 - g_0|$,  $M(i, -1) = M(-1, j) = 1/\epsilon$,
%%where
%%\begin{equation*}
%%	d(f_i, g_j) = \max(|t_i - t_j|, |f_i - g_j|).
%%\end{equation*}
%%
%%As a result, 
%such that $M(2n, 2n)$ is the Skorokhod distance of $f$ and $g$ on $[t_0, t_n]$.

\subsection{Initial density vanishing at zero and no discontinuity}\label{sim1/2}

We first consider an example with $\lim_{x\downarrow0} f(x)=0$. % and there is no discontinuity in $\Lambda$ observed.
%, and demonstrate the convergence of the method in Skorokhod metric. 
To this end, we let $X_{0-}$ be $\Gamma(3/2,1/2)$-distributed and note that $f(x)\le Cx^{1/2}$, $x\ge0$ for a suitable constant $C<\infty$. Further we fix the time interval $[0,T]=[0,0.8]$ and $\alpha = 1.3$.
%{\color{blue} \fbox{What is $\beta$? 1/2?}}

%We perform numerical simulations using Algorithm 1 from \cite{KR} on a uniform grid. 
In Figure 1(a), we exhibit $L^{0.8/n}$ on the time interval $[0,0.8]$ for different numbers $n$ of time steps (or equivalently different values of $\Delta=0.8/n$). The numerical simulations indicate that there is no discontinuity in this setting.

\captionsetup[subfigure]{labelfont=rm}

\begin{figure}[h]
	\begin{center}
		%\subfloat[]{\includegraphics[width=0.55\textwidth]{loss_gamma05.eps}}
		\subfloat[]{\includegraphics[width=0.5\textwidth]{ex1.eps}\label{fig:example1a}}
		\subfloat[]{\includegraphics[width=0.5\textwidth]{mc_error_sup_05.eps}\label{fig:example1b}} \\
	\end{center}
	%\vspace{-5pt}
	\caption{Example with $\lim_{x\downarrow0} f(x)=0$ and no discontinuity for different values of $n$: (a) absorption probabilities $L^{0.8/n}_t=\Lambda^{0.8/n}_t/1.3$, $t\in[0,0.8]$, and (b) error in the supremum norm over the time interval $[0,0.8]$.}
 	\label{fig:example1}
\end{figure}	

We approximate the error in the supremum norm by %$d_{\text{M1}}(L_T^{T/n}, \bar{L}_T)$, 
$\sup_{t\in [0,0.8]} |L_t^{0.8/n} - \bar{L}_t|$,
where a reference solution $\bar{L}:=L^{0.8/\bar{n}}$ is computed on a refined time mesh with $\bar{n} = 25600$ points.
 %, and $d(\cdot, \cdot)$ is the Skorokhod distance. 
The convergence rate suggested by Figure 1(b) is around 0.5, as confirmed visually by a comparison with a reference line (on the log-scale) of slope $-0.5$. This is expected from Remark \ref{rm_order}(a) and has been also observed in \cite[Section 4.2]{KR} for the pointwise error. We note that the two rightmost data points deviate slightly from the predicted line due to the comparison with a reference solution computed on a refined time mesh. Accordingly, the convergence order estimated by regression is slightly biased high, namely 0.55.

\subsection{Initial density of $1/\alpha$ at zero and no discontinuity}\label{sec5.3}

We turn to the numerical examination of the rate of local convergence when $\lim_{x\downarrow0} f(x)=\frac{1}{\alpha}$ (cf.~Theorem \ref{thm:loc_conv})
%Proposition \ref{prop:loc_conv}
and illustrate that the rate may indeed be arbitrarily low. % due to a discontinuity. 
%To this end, we pick the initial density
%\begin{equation}
%\label{dens_a_alph}
%	f(x) = \left\{
%	\begin{tabular}{ll}
%		$\frac{1}{\alpha} - x^{a}$, & \quad $0 \le x \le \alpha^{-1/a}$, \\
%		$\frac{2}{\alpha}$, & \quad $\alpha^{-1/a}<x\le A$, \\
%		$0$, & \quad $x > A$,
%	\end{tabular} \right.
%\end{equation}
%for $\alpha\ge1$ and $a>0$, which we vary in the tests, and where $A> \alpha^{-1/a}$ is such that $\int_0^\infty f(x)\,\mathrm{d}x=1$. This choice corresponds to taking $\psi(x)=x^a$ and $\Psi(x)=x^{a+1}/(a+1)$ in Theorem \ref{thm:loc_conv}.
To this end, we pick the initial density
\begin{equation}
\label{dens_a_alph}
	f(x) = \left\{
	\begin{tabular}{ll}
		$\frac{1}{\alpha} - c x^{a}$, & \quad $0 \le x \le A$, \\
		$0$, & \quad $x > A$,
	\end{tabular} \right.
\end{equation}
for $\alpha>0$ and $a>0$, which we vary in the tests, and where $A>0$ is determined by $\int_0^\infty f(x)\,\mathrm{d}x=1$ for given $c>0$, the latter being sufficiently small. This choice corresponds to taking $\psi(x)=c x^a$ and $\Psi(x)=c x^{a+1}/(a+1)$ in Theorem \ref{thm:loc_conv}.
%Propositions \ref{prop:density_est} and \ref{prop:loc_conv} 
%Assuming the last term in \eqref{loc_rate_conv} to be the dominant one, we expect a convergence rate of $1/(2(a+1))$ independent of $\alpha$.
%Using such a choice of the initial density, 
%This example is constructed in a way that the value of the density near $x=0$ is close to $\frac{1}{\alpha}$, the critical value in Theorem \ref{thm1}. 
Moreover, we let $T=10^{-4}$ be small enough to precede a possible discontinuity. %, and fix again $N = 10^7$ particles.
%As in the previous example, we compute the infinity norm error for varying $n$ between $L^{T/n}$ and $\overline{L}$, the solution computed with $n=\bar{n} = 25600$. %, on $[0,T]$.

\medskip

To exhibit the rate of convergence we plot in Figure \ref{fig:example2new} the error in the supremum norm as a function of the number $n$ of time steps on a log-log scale, for $\alpha\in\{0.5,1\}$ and $a\in\{1, 2, 4\}$. (We also adjust the constant $c$ for each $\alpha$ and $a$.)
%(For $a \in \{1, 2\}$, we took $c = 1/10$, whereas for $a = 4$ we used $c = 1/100$.)
These errors are compared to the reference line of slope $-1/(2(a+1))$, which reflects the term on the second line in \eqref{roc}.
%\footnote{The last data points deviate slightly from the predicted line due to comparison with the reference solution, which is computed on a further refined mesh.}
\begin{figure}[h]
	\begin{center}
		%\subfloat[]{\includegraphics[width=0.55\textwidth]{loss_gamma05.eps}}		
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a1alpha05.eps}\label{fig:a1alpha05}}
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a1alp1.eps}\label{fig:a1alpha1}} \\
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a2alp05.eps}\label{fig:a2alpha05}}
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a2alp1.eps}\label{fig:a2alpha1}} \\
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a4alp05.eps}\label{fig:a4alpha05}}
		\subfloat[]{\includegraphics[width=0.5\textwidth, height=0.3\textwidth]{a4alp1.eps}\label{fig:a4alpha1}}
	\end{center}
	\caption{Error in the supermum norm over $[0,10^{-4}]$ for the initial densities of \eqref{dens_a_alph} with: (a) $a=1$, $\alpha=0.5$, (b) $a=1$, $\alpha=1$, (c) $a=2$, $\alpha=0.5$, (d) $a=2$, $\alpha=1$, (e) $a=4$, $\alpha=0.5$, and (f) $a=4$, $\alpha=1$. We showcase the error for different $n$, and a reference line of slope $-1/(2(a+1))$.
	}
 	\label{fig:example2new}
\end{figure}	
The data for most parameter pairs suggest a convergence of polynomial order consistent with that term. As already pointed out in Remark \ref{rm_order}(b), the asymptotically dominant term on the right-hand side of \eqref{roc} is the first, logarithmic one, indicating that the theoretical result may not be sharp. The rate appears independent of $\alpha$, but the constant of proportionality of the error seems to be affected by it when one contrasts the errors in the respective left and right plots. The last two plots, for $a=4$ and $\alpha \in \{0.5,1 \}$, are less well explained by this. We find the convergence for large $a$ to be extremely slow, which may explain why the true asymptotic order is not detected for computationally feasible numbers of particles and time steps. %Note that $1-x^4/100$ is very close to 1 for small $x$.

\medskip

We also show in Table \ref{table:convergence_rate}, for varying values of $\alpha$ and $a$, the convergence rate estimated by regression from the logarithmic errors in the supremum norm for $n=25,\,50,\,\ldots,\,800$. The estimated rates are mostly independent of $\alpha$, and in many cases close to $1/(2(a+1))$, this being the rate suggested by the term on the second line in \eqref{roc}. Some significant deviations are again found for larger $a$ and $\alpha$, which may again be due to the large errors in such cases.
%\begin{table}[H]
%	\begin{center}
%	\begin{tabular}{| c | c | c | c | c | c | c |}
%  \hline			
%$a \backslash \alpha$ & 1/(2($a$+1)) &   0.1 & 0.5 & 1.0 & 1.5\\
% \hline
%1 & 1/4 = 0.25 &   0.21 & 0.21 & 0.22 & 0.4\\
%2 & 1/6 $\approx$ 0.17 &  0.15 &0.15 & 0.15 & 0.16\\
%4 & \!\!\!\!\!\!\!\! 1/10 = 0.1 &  0.12 & 0.11 & 0.08 & 0.08\\
%8 & 1/18 $\approx$ 0.055 &  0.05 & 0.04 & 0.04 & 0.05 \\
%16 & 1/34 $\approx$ 0.029 &  0.03 & 0.03 & 0.06 & 0.06 \\ \hline
%\end{tabular}
%\caption{Convergence rate for different values of $a$ and $\alpha$ with $T = 10^{-4}$.}
%\label{table:convergence_rate}
%\end{center}
%\end{table}
%\begin{table}[H]
%	\begin{center}
%	\begin{tabular}{| c | c | c | c | c | c | c |}
%  \hline			
%$a \backslash \alpha$ & 1/(2($a$+1)) &   0.1 & 0.5 & 1.0 & 1.5\\
% \hline
%1 & 1/4 = 0.25 &   0.25 & 0.27 & 0.29 & 0.27 \\
%2 & 1/6 $\approx$ 0.17 &  0.20 &0.18 & 0.20 & 0.18 \\
%4 & \!\!\!\!\!\!\!\! 1/10 = 0.1 &  0.099 & 0.10 & 0.13 & 0.25 \\
%8 & 1/18 $\approx$ 0.056 &  0.057 & 0.053 & 0.081 & 0.13 \\ \hline
%\end{tabular}
%\vspace{15pt}
%\caption{Estimated convergence rates on the time interval $[0,10^{-4}]$ for different values of $a$ and $\alpha$.}
%\vspace{-20pt}
%\label{table:convergence_rate}
%\end{center}
%\end{table}
%a = 1, alpha = 0.5: 0.2593
%a = 1, alpha = 1: 0.2617
%a = 2, alpha = 0.5: 0.1746
%a = 2, alpha = 1: 0.1804
%a = 4, alpha = 0.5: 0.1248
%a = 4, alpha = 1: 0.1011
\begin{table}[H]
	\begin{center}
	\begin{tabular}{| c | c | c | c | c | c | c |}
  \hline			
$a \backslash \alpha$ & 1/(2($a$+1)) &   0.1 & 0.5 & 1.0 & 1.5\\
 \hline
1 & 1/4 =  0.25 & 0.234  & 0.259 & 0.261 & 0.261 \\
2 & 1/6 $\approx$ 0.17 & 0.169 &0.175 & 0.180 & 0.166  \\
4 & \!\!\!\!\!\!\!\! 1/10 = 0.1 &  0.104 & 0.125 & 0.101 & 0.089 \\
8 & 1/18 $\approx$ 0.056 & 0.053 & 0.049 & 0.025 & 0.033 \\ \hline
\end{tabular}
\vspace{15pt}
\caption{Estimated convergence rates on the time interval $[0,10^{-4}]$ for different values of $a$ and $\alpha$.}
\vspace{-20pt}
\label{table:convergence_rate}
\end{center}
\end{table}
%alpha = 0.1
%a = 1: 0.2494
%a = 2: 0.2011
%a = 4: 0.0993
%a = 8: 0.0570
%
%alpha = 0.5
%a = 1: 0.2670
%a = 2: 0.1802
%a = 4: 0.1041
%a = 8: 0.0532
%
%alpha = 1.0
%a = 1: 0.2891
%a = 2: 0.2001
%a = 4: 0.1346
%a = 8: 0.0811
%
%alpha = 1.5
%a = 1: 0.27
%a = 2: 0.18
%a = 4: 0.25
%a = 8: 0.13

\subsection{ %H\"{o}lder $1/2$ initial data and 
Example with discontinuity} 

In our last example, we study a scenario with a discontinuity. We consider the same setting as in Subsection \ref{sim1/2}  except that we choose $\alpha = 1.5$ and $T = 0.008$. In this case, we suspect from Figure \ref{fig:example2} a discontinuity of the true physical solution around $t = 0.002$. 
\vspace{-13pt}
\begin{figure}[h]
	\begin{center}
		%\subfloat[]{\includegraphics[width=0.55\textwidth]{loss_gamma05.eps}}
		%\subfloat[]
		\includegraphics[width=0.7\textwidth,height=0.45\textwidth]{ex2.eps}%\label{fig:example2a}
		%		\subfloat[]{\includegraphics[width=0.5\textwidth]{Figures/ex2_errr.eps}\label{fig:example2b}} \\
	\end{center}
	\vspace{-17pt}
	\caption{Absorption probabilities $L^{0.008/n}_t=\Lambda^{0.008/n}_t/1.5$ for varying $n$.}
	%Example with H\"{o}lder $1/2$ initial data and discontinuity for different $n$: (a) Loss function $L^{T/n}_t=\Lambda^{T/n}_t/\alpha$; (b) Skorokhod error on $[0,T]$.}
	\label{fig:example2}
\end{figure}
\vspace{-7pt}
The numerical approximations approach the discontinuity ``from the right'' as $\Delta\downarrow 0$, which reflects how larger time steps slow down the build-up of the probability mass close to the origin and hence delay the onset of the blow-up. By the mechanism revealed in our key Lemma \ref{lem:jump-dens}, however, for small enough $\Delta>0$, the probability of the numerical solution being close to the origin is nearly that of the physical solution just before the blow-up time of the latter, and then, by Lemma \ref{lem::special_case}, the numerical solution catches up with the discontinuity after a short time.

Figure \ref{fig:example2} also explains the choice of the M1 topology in Theorem \ref{thm::main}, rather than the J1 or the supremum norm topology (see \cite[Section 3.3]{Whi}, \cite[Appendix A.1]{CRS} for juxtapositions of these topologies), as the numerical solution seems to approach the discontinuity by many small jumps.  

We are unable to make any general claims about the rate of convergence in the blow-up regime, and therefore do not estimate it numerically. Instead, we refer the interested reader to \cite[Section 4.3]{KR} for further numerical illustrations of the convergence in this regime. %, including the time of the discontinuity, the $L_1$ distance, and the inverse map $t \rightarrow L_t^{-1}$.

%In this example, from Figure \ref{fig:example2b} it remains unclear whether there is a positive convergence order for the numerical approximations. % in the .
%suggests that our method still gives convergence in the Skorokhod topology,
%and the order of convergence remains $0.5$ on average over the refinements considered, but appears asymptotically lower. %We investigate this phenomenon in detail in the following section.
%but it remains unclear whether there is a positive order.

%\vspace{-20pt}


==> arXiv v2/include.tex <==
\usepackage{amsmath, amssymb, amsthm}
\usepackage{setspace}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{pdfpages}
\usepackage{listings}
\usepackage{bbm}
\usepackage{hyperref}
\usepackage{subfig}
\usepackage{color}
\usepackage{float}
\usepackage{amssymb}

\usepackage{cancel}

\newcommand{\chr}[1]{{\color{blue} #1}}
\newcommand{\chrb}[1]{{\color{blue} \fbox{#1}}}

\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\Var}{Var}

\DeclareMathOperator{\xx}{\mathbf{x}}
\DeclareMathOperator{\yy}{\mathbf{y}}


\DeclareMathOperator{\XX}{\mathbf{X}}
\DeclareMathOperator{\YY}{\mathbf{Y}}
\DeclareMathOperator{\BCC}{\mathbb{C}}
\DeclareMathOperator{\BEE}{\mathbb{E}}
\DeclareMathOperator{\BII}{\mathbb{I}}
\DeclareMathOperator{\BNN}{\mathbb{N}}
\DeclareMathOperator{\BPP}{\mathbb{P}}
\DeclareMathOperator{\BQQ}{\mathbb{Q}}
\DeclareMathOperator{\BRR}{\mathbb{R}}
\DeclareMathOperator{\BTT}{\mathbb{T}}
\DeclareMathOperator{\BZZ}{\mathbb{Z}}
\DeclareMathOperator{\BONE}{\mathbbm{1}}
\DeclareMathOperator{\CBB}{\mathcal{B}}
\DeclareMathOperator{\CCC}{\mathcal{C}}
\DeclareMathOperator{\CFF}{\mathcal{F}}
\DeclareMathOperator{\CII}{\mathcal{I}}
\DeclareMathOperator{\CLL}{\mathcal{L}}
\DeclareMathOperator{\CSS}{\mathcal{S}}
\DeclareMathOperator{\CTT}{\mathcal{T}}

\DeclareMathOperator{\OSS}{\overline{S}}
\DeclareMathOperator{\USS}{\underline{S}}


\DeclareMathOperator{\La}{\Lambda}

\DeclareMathOperator{\veps}{\varepsilon}
\DeclareMathOperator{\vphi}{\varphi}

\DeclareMathOperator{\boldalpha}{\boldsymbol{\alpha}}
\DeclareMathOperator{\boldbeta}{\boldsymbol{\beta}}
\DeclareMathOperator{\boldlambda}{\boldsymbol{\lambda}}
\DeclareMathOperator{\boldpi}{\boldsymbol{\pi}}
\DeclareMathOperator{\boldomega}{\boldsymbol{\omega}}

\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

